Backdoor Attacks and Defenses in Federated Learning: Survey, Challenges and Future Research Directions

Federated learning (FL) is a machine learning (ML) approach that allows the use of distributed data without compromising personal privacy. However, the heterogeneous distribution of data among clients in FL can make it difficult for the orchestration server to validate the integrity of local model updates, making FL vulnerable to various threats, including backdoor attacks. Backdoor attacks involve the insertion of malicious functionality into a targeted model through poisoned updates from malicious clients. These attacks can cause the global model to misbehave on specific inputs while appearing normal in other cases. Backdoor attacks have received significant attention in the literature due to their potential to impact real-world deep learning applications. However, they have not been thoroughly studied in the context of FL. In this survey, we provide a comprehensive survey of current backdoor attack strategies and defenses in FL, including a comprehensive analysis of different approaches. We also discuss the challenges and potential future directions for attacks and defenses in the context of FL.

==> assessment.tex <==
\subsection{Evaluation Metrics}
% Since the attacking objective of the adversary is to mislead the global model to misbehave on the backdoored inputs (i.e., the global model classifies the images of ``green car" as ``frog" in image classification task).
% Therefore, the matrices to measure the efficiency of a backdoor attack are necessarily associated with the objective of the backdoor attack.
% The first metric, named attack success rate (ASR), which measures the probability that the outputs of backdoored model given targeted inputs are similar to the adversary's preference.
% Other terms such as backdoor task accuracy ~\citep{wang2020attack}, poisoning accuracy ~\citep{?} refers to the same meaning as ASR. Technically, the higher backdoor accuracy is, the higher attack success rate is.
The objective of an adversary's backdoor attack is to mislead the global model to produce incorrect outputs on backdoored inputs (e.g., the global model classifies images of "green cars" as "frogs" in an image classification task). Therefore, the metrics used to evaluate the effectiveness of a backdoor attack are related to the attack's objective. One metric, called attack success rate (ASR), measures the probability that the output of the backdoored model on targeted inputs matches the adversary's preference. Other term such as backdoor task accuracy~\citep{wang2020attack} refers to the same concept as ASR. In general, a higher backdoor accuracy corresponds to a higher attack success rate.

Mathematically, let $\tilde{\mathbf{\mathcal{D}}}$ be the targeted samples (e.g., images inserted trigger pattern), and the $\tau$ be the targeted class of the adversary. Since the backdoored model $\mathbf{f}_{\textbf{W}}$ is expected to misclassify $\tilde{\mathbf{\mathcal{D}}}$ as $\tau$, the ASR is calculated by:
\begin{equation}
    \text{ASR} = \sum_{x\in \tilde{\mathbf{\mathcal{D}}}} \frac{ \mathbf{f}_{\mathbf{W}}(x) = \tau}{| \tilde{\mathbf{\mathcal{D}}} |}
\end{equation}

Additionally, the trained model $\mathbf{f}_{\textbf{W}}$ should produce normal outputs on benign samples (e.g., images without triggers). The model's accuracy on these samples can be measured using the metric called main task accuracy (MTA) on benign samples. This is calculated as:
\begin{equation}
    \text{MTA} = \sum_{x_i\in \mathbf{\mathcal{D}}} \frac{ \mathbf{f}_{\mathbf{W}}(x_i) = y_i}{| \mathbf{\mathcal{D}} |},
\end{equation}
where $\mathbf{\mathcal{D}} := \left[ x_1^{y_1}, x_2^{y_2}, \dots,  x_{|\mathbf{\mathcal{D}}|}^{y_{|\mathbf{\mathcal{D}}|}}\right]$  is the validation set held by the aggregator, and $y_i$ is the corresponding label for sample $x_i$. In most backdoor attack strategies, the adversary is successful in planting the backdoor only if the trained model has both high MTA and significant ASR~\citep{bagdasaryan2020backdoor,wang2020attack}. A simple illustration of these two common metrics is shown in Figure~\ref{fig:backdoor-metrics}.
% In the meantime, the trained model $\mathbf{f}_{\textbf{W}}$ needs to behave normally on the benign samples (e.g., other images without the trigger). Let denote $\mathbf{\mathcal{D}} := \left[ x_1^{y_1}, x_2^{y_2}, \dots,  x_{|\mathbf{\mathcal{D}}|}^{y_{|\mathbf{\mathcal{D}}|}}\right]$ as the validation set that the the aggregator may hold, then the MTA is expressed as:
% \begin{equation}
%     \text{MTA} = \sum_{x_i\in \mathbf{\mathcal{D}}} \frac{ \mathbf{f}_{\mathbf{W}}(x_i) = y_i}{| \mathbf{\mathcal{D}} |},
% \end{equation}
% where $y_i$ is the corresponding label for sample $x_i$. In most of backdoor attack strategies, the adversary conducts implanting backdoor attack successfully if and only the trained model has high MTA and significant ASR~\citep{bagdasaryan2020backdoor,wang2020attack}. The simple illustration for the two common metrics are presented in Figure~\ref{fig:backdoor-metrics}.

\begin{figure*}[tb]
    \centering
\begin{minipage}{0.5\textwidth}
% \includegraphics[width=\columnwidth]{figures/by_class_grad.eps}
	\centering\includegraphics[width=1.0\textwidth]{figures/backdoor_metrics.pdf} % Reduce the figure size so that it is slightly narrower than the column.
% 	\vspace{-0.8em}
	\caption{Common metrics for backdoor attacks and defenses.}
	\label{fig:backdoor-metrics}
\end{minipage}
\hfill
% \begin{minipage}{0.4\textwidth}
% 	\centering\includegraphics[width=1.0\textwidth]{figures/hfl-pipeline.pdf} % Reduce the figure size so that it is slightly narrower than the column.
% % 	\vspace{-0.8em}
% 	\caption{General threat model of backdoor attack on HFL.}
% 	\label{fig:backdoor-hfl}
% \end{minipage}
\end{figure*}
To evaluate the effectiveness of FL defenses against backdoor attacks, ASR and MTA which are mentioned above are widely used. In most existing defenses, the authors aimed at minimizing the ASR while not degrading the MTA. In addition, in the anomaly detection-based defenses, other metrics are employed to evaluate the accuracy in detecting malicious updates~\cite{nguyen2022flame}. In particular, they measure true positive rate (TPR) and true negative rate (TNR), which are defined as follows.
\begin{itemize}
    \item \textbf{TPR: }measures how well the defense identifies poisoned models, e.g., the ratio of the number of models correctly classified as poisoned (True Positives - TP) to the total number of models being classified as poisoned: $TPR = \frac{TP}{TP+FP}$, where FP is False Positives indicating the number of benign clients that are wrongly classified as malicious.
    \item \textbf{TNR:} measures the ratio of the number of models correctly classified as benign (True Negatives - TN) to the total number of benign models: $TNR = \frac{TN}{TN+FN}$, where FN is False Negatives indicating the number of malicious clients that are wrongly classified as benign.
\end{itemize}

% \subsection{Backdoor Attacks in Different FL Schemes}
% \input{tables/backdoor-attack-proposals}
% \input{tables/backdoor-attack-dimension}

% \subsubsection{Horizontal Federated Learning}

% We first compare the existing attacks in the following eight dimensions in Table~\ref{tab:backdoor-attack-comparision}. Then, we explain in detail each dimension considered to compare in Table~\ref{tab:attack-dimension}.

% \noindent\textbf{Backdoor Characteristics. }
% Most of state-of-the-art attacks follow the common attack strategy which combines data poisoning and model poisoning to intensify the backdoor effect. For example, as reported in~\citep{Xie2020DBADB}, the distributed backdoor attack without scaling achieve low attack success rate (i.e., below 5\%); meanwhile, using scale factor wisely can boost the ASR to approximately 100\%. Other attack with solely data poisoning requires the continuous attack to achieve successfully backdoor effect (i.e., the malicious partipants are selected in multiple rounds). For instance, in~\cite{wang2020attack}, with the assumption that one malicious client can join the FL training every 10 rounds, the adversary can achieve almost 80\% of backdoor task accuracy in digit classification on EMNIST. The attack which requires only data poisoning is easy to conduct for even non-tech adversary with limited capability and knowledge about the training protocol as well as aggregation operator.

% \noindent\textbf{Adversary Capability. }
% In addition to the adversary's in common threat model, authors in~\citep{PoisonGAN,SemiTargetedMP-Sun2022,Liu2022TechnicalRA} proposed using customized local training mechanism instead of simply varying number of local epochs or training parameters, i.e., training additional GAN network to generate poisoning samples in alignment with the data population of the benign clients \citep{PoisonGAN}.\\
% To conduct effective backdoor attack, the participant collusion is employed. The higher colluding ratio, the stronger attack (cf.~\citep{Sun2019CanYR}). As a result, the backdoor durability is also increased when the adversary owns large number of compromised clients. However, the malicious clients often account for just a small portion among total clients in practical scenario, i.e., $\left[0.01, 1\right]\%$ (cf.~\citep{Shejwalkar2021BackTT}). Therefore, the assumption about the large ratio of malicious participants may not be hold. In most of the proposed attacks~\citep{fung2018mitigating,wang2020attack,Xie2020DBADB,Nguyen2020PoisoningIoT}, the malicious clients are assumed to participate in multiple training rounds, i.e., continuous attack. However, this kind of attack may not be hold practically since the number of participants randomly selected in each training round is much more smaller than total clients, which means the probability that an adequate ratio of $\mathcal{M}$ joining training is very small. The direct solution for this is an effective single-shot attack~\citep{bagdasaryan2020backdoor,Liu2022TechnicalRA}. This approach seems practical since each malicious client may be selected only once in the large-scale FL system (cf.~\citep{Shejwalkar2021BackTT}).

% \noindent\textbf{Attack efficiency. }
% The efficiency of an attack is evaluated under three key dimensions: stealthiness, durability and flexibility. \\
% \noindent One of the biggest challenges to backdoor attack designing is that the malicious clients often account for just a small portion among total clients in reality, i.e., $\left[0.01, 1\right]\%$ (cf.~\citep{Shejwalkar2021BackTT}). Therefore, the poisoned updates may be easily diluted by the benign updates. This phenomenon is also known as ``catastrophic forget" in machine learning. The techniques aim to replace the global model with the poisoned one~\citep{bagdasaryan2020backdoor} or continuously remind the global model about the backdoor task by continuous participation of malicious clients~\citep{Xie2020DBADB} can prolong the backdoor effect. Another approach tried to implant backdoor into the neurons which are least overlapped with the active neurons for the main task by employing the rare samples~\citep{rare-Yoo2022BackdoorAI,wang2020attack}. More recently, the durability of the backdoor is more seriously taken into account in~\citep{Neurotoxin,Liu2022TechnicalRA,Zhou2021DeepMP} and this opens a new novelty to design a robust and durable backdoor attack. \\
% \noindent Conspicuous backdoor attack is hard to be practical since the various defenses available for aggregation server. It is trivial that the scaled malicious updates may have abnormally large values compared to the benign ones, which may easily detected.

% Realizing this fact, many approaches consider utilizing additional techniques together with scaling the poisoned updates to make the backdoor more resistant against a range of defense mechanisms (i.e., PGD attack~\citep{Sun2019CanYR}, constrain-and-scale~\citep{wang2020attack}). However, whether these techniques are robust against state-of-the-art defense mechanisms is still an open question. \\
% The flexibility of a backdoor attack strategy is an important factor to be considered in real-world scenario. Therefore, an attack should not depend on many constraints such as training stage (i.e., early training rounds or converged training rounds), number of malicious participants, etc.

% \subsubsection{Vertical Federated Learning}
% \begin{figure}[tbh]
%      \centering
%      \includegraphics[width=0.6\textwidth]{figures/backdoor-vfl.pdf}
%      \caption{\textbf{A common backdoor attack scheme in Vertical FL.}}
%      \label{fig:vfl_attack_pipeline}
%  \end{figure}
% Due to the difference in the mechanism between Horizontal FL and Vertical FL, the attack strategy is varied. The following attack scheme is considered:  (i) the attacker has access to the training data of one or more data parties $D_m$ and it controls the training procedure and local hyperparameters of attacked parties. (ii) The attacker can modify local updates such as training weight and gradients before sending transmitted data to other parties. (iii) The attacker does not control any benign parties’ training nor does the attacker control the global communication and aggregation protocols. (iv) Contrary to traditional data poisoning attacks which focus on poisoning training data, the attacker in collaborative learning focus on poisoning gradients and model updates that are communicated among parties in the protocol.
% The main difference between backdoor attacks on Horizontal FL and Vertical FL is that: in VFL, the attacker only has access to a portion of the feature space of parties that it controls, and it may not have access to labels if it doesn’t control the active party. Moreover, it also has only a portion of the model parameters of the parties it controls.

% VFL is under-studied for the lack of datasets and benchmarks~\citep{Cai2022AcceleratingVF}, so there are not so much effort put for the backdoor attack on VFL. To the best of our knowledge,~\cite{Liu2021BatchLI-VFL} first introduced \textit{Gradient-replacement backdoor} by wisely swap the gradients of benign and poisoned samples before sending back to the active party. This method is proved to be effective in the later work~\citep{Zou2022VFL} even when the communication between parties in FL is protected by Homomorphic encryption (HE)~\citep{HE2020}.


\subsection{Confrontation between Backdoor Attacks and Defenses}
\input{tables/backdoor-link-attack-defense}
% \textcolor{red}{TODO}
% \input{tables/attack-defense-assessment}
% \textcolor{blue}{One key observation from Table \ref{tab:stat-defen} is that some of the backdoor defense mechanisms only work when the number of malicious clients is large enough. For example,~\cite{Nguyen2022-FLAME, rieger2022deepsight, li2020learning, sun2021fl} proposed defense methods that required a large percentage of malicious clients (up to 50\%) to be present in order to effectively detect and exclude them. This highlights the importance of understanding the specific threat model and the distribution of malicious clients in a given scenario.}

% \textcolor{blue}{Another key observation is that most of the defense mechanisms need access to the global model in order to exclude or reduce the impact of backdoor updates. However, some defense mechanisms access the inference from local data, which can be time-consuming for clients. For example,~\cite{rieger2022deepsight, andreina2021baffle} proposed a defense method that required clients to perform additional local computations to detect backdoor updates, which can increase the communication and computation overhead for clients. It is important to balance the trade-offs between the overhead and the effectiveness of the defense mechanisms when selecting a defense method for a specific scenario.}

Adversaries and defenders are engaged in a never-ending battle. The conflict between them deepens our understanding of backdoor attacks. Attackers are always looking for ways to make poisoned attacks more covert, effective, and resistant to countermeasures. As shown in Table~\ref{tab:stat-attack-defense}, most defense strategies focus on the scenarios of in-distribution backdoor attacks, in which the adversary simply changes the label of targeted inputs into his expected one. These poisoned samples can appear in the other benign participants' training data. Although defense is often designed against multiple attacks, many attack strategies have not been addressed such as noise-instance, coordinated-trigger, and partially poisoning backdoor attacks.

% The primary objective for defenders is to successfully thwart as many kinds of unexpected backdoor attacks as possible. We summarize attack strategies and the corresponding applicable defenses in Table~\ref{tab:stat-attack-defense}. 


On the other hand, each countermeasure approach is often applied to a group of attack strategies. Particularly, pre-aggregation methods (e.g., Krum, FoolsGold, and AUROR) seem to be efficient under semantic backdoor attacks. Furthermore, in--aggregation methods are primarily utilized under artificial backdoor attacks, specifically single-trigger attacks. However, the more sophisticated attack strategies such as distributed-trigger and coordinated-trigger, have not been evaluated under the presence of these defenses.


==> backdoor-attack-taxonomy.tex <==
The backdoor attack is first introduced in FL by Bagdasaryan et al.~\cite{HTBD2018}. Since then, backdoor attacks have received widespread attention and became the primary security threat in FL. In most existing works~\cite{wang2020attack,2021-AdvancesOPFL,Nguyen2022-FLAME,RODRIGUEZBARROSO2022-FL-threat-survey,Neurotoxin}, backdoor attacks are categorized into two classes: \textbf{data poisoning attack} and \textbf{model poisoning attack} with respect to different attack stages: training data collection and local training procedures. The goal of the former is to manipulate a poisoned training dataset in order to corrupt the corresponding local model, while the latter aims at altering a poisoned model to enhance the attack's effectiveness. In this study, we introduce more taxonomies from the perspectives of adversarial goals and backdoor application scope. 

Regarding the purposes of backdoor attacks, FL backdoor attacks can be classified into \textbf{semantic backdoor attack} and \textbf{artificial backdoor attack}. In semantic backdoor attacks, the targeted inputs should have specific properties, e.g., a pixel pattern or a word sequence, e.g., cars with striped pattern~\cite{bagdasaryan2020backdoor}. 
In this category of attack, no modification is conducted to modify the features of backdoored samples. On the other hand, artificial backdoor attacks~\cite{Xie2020DBADB,HTBD2018,Gong2022CoordinatedBA} aim to misclassify any poisoned input containing a backdoor trigger. Note that, these backdoored samples are created by artificially inserting triggers into the clean inputs. In the testing phase, the semantic backdoor attack can prompt misbehavior without any modification on the input samples while an artificial backdoor attack needs additional interference to manipulate targeted samples.

In the following sections, we will present detailed introductions to these backdoor attack techniques. We compare the state-of-the-art attack strategies in Table~\ref{tab:backdoor-attack-comparision}.
% based on eight dimensions and explain each dimension in Table~\ref{tab:attack-dimension}.

\input{tables/backdoor-attack-proposals.tex}
% \input{tables/backdoor-attack-dimension}
% Note that, such test inputs should be modified to incorporate the backdoor trigger into inputs and only the adversary or a malicious client know the trigger. 
% It is worth noting that semantic backdoor attack covers the term ``physical backdoor attack" well-known in ML~\citep{Wenger2021PhysicalBA} to some extend. In specific, physical backdoor attack leverages the physical objects as triggers, thus making them a credible threat against deep learning systems, i.e., the trigger is ``white tape" on the forehead in the face recognition task. To achieve his goal, the adversary often manipulates the poisoning data of one or many compromised clients. However, the method to manipulate the poisoned training data that the adversary leverages vary significantly and could be roughly classified into three main approaches as follows.
% which is clearly presented via the characteristic of the targeted samples that the attacker leads the model to mis--classify



==> backdoor_attack.tex <==
% \subsection{Taxonomy and description}
\begin{figure*}[tbh]
     \centering
     \includegraphics[width=0.7\linewidth]{figures/taxonomy-backdoor.pdf}
     \caption{\textcolor{purple}{\textbf{Taxonomy of FL backdoor attacks}}}
     \label{fig:backdoor_attack_taxonomy}
 \end{figure*}
There are many significant dimensions associated with a backdoor attack strategy, which are depicted in Tab. \ref{tab:backdoor-attack-comparision}. Based on different criteria, a number of ways to categorize backdoor attacks in FL were proposed. In particular, authors in ~\cite{wang2020attack},~\cite{2021-AdvancesOPFL},~\cite{Nguyen2022-FLAME},~\cite{RODRIGUEZBARROSO2022-FL-threat-survey},~\cite{Neurotoxin} mentioned \textit{Data Poisoning} and \textit{Model Poisoning} as two main taxonomies of backdoor attack in FL, which characterizes for the two manners of inserting backdoor. This approach is known as the most widely-used way to categorize the backdoor attack in the literature. On the other hand, ~\cite{Shejwalkar2022-BackDB},~\cite{bagdasaryan2020backdoor} divided backdoor attacks on FL into \textit{Semantic backdoor attack} and \textit{Artificial backdoor attack} or \textit{Pixel backdoor attack} based on the discriminate property of the backdoor inserted. Along with the line,~\cite{wang2020attack} introduced \textit{Black-box attack} and \textit{White-box} attack, which is representative for the capability of the attacker. Moreover, many other perspectives are employed to classify backdoor attack on FL such as: attack frequency~\cite{bagdasaryan2020backdoor}, distributed property~\cite{Liu2022-EvilvsEvil}, etc.

In our work, we follow the majority of previous studies and roughly classify the backdoor attack strategies in FL into two primary categories: \textbf{Data poisoning attack} and \textbf{Model poisoning attack}. This systemizing approach is associated with two sub-phases of the FL training pipeline in, which are training data collection and learning procedure. Training data collection is to gather a training dataset, and the learning procedure generates a model based on the training dataset. From this, further categories are studied based on the different techniques to implant the backdoor. The taxonomies of backdoor attacks in FL are summarized in Figure~\ref{fig:backdoor_attack_taxonomy}.
\subsection{Data Poisoning}
In data poisoning attacks, it is assumed that the adversary has complete control over the training data collection process of compromised clients. In particular, the adversary manipulates the training data such that, following the completion of the local training procedure, any compromised client's local update is poisoned. Most of the time, the poisoned training dataset has both clean samples and a subset of data with a backdoor trigger. Interestingly, the purposes of the attacker when trying to insert the backdoor are different, which is clearly presented via the characteristic of the targeted samples that the attacker leads the model to misclassify. Based on this point, data poisoning attack is further classified into \textit{semantic backdoor} and \textit{artificial backdoor attacks}.\\

\subsubsection{Semantic backdoor. }The attacker employs semantic backdoor targets at misleading the aggregated model to classify a set of samples with the specific properties as his targeted label (e.g., cars with certain attributes are classified as birds~\cite{bagdasaryan2020backdoor}). In this category of attack, the key of the backdoor is ``input-instance" and no modification is necessary on the features of backdoored samples. It is worth noting that semantic backdoor attack covers the term ``physical backdoor attack" well-known in ML~\citep{Wenger2021PhysicalBA} to some extend. In specific, a physical backdoor attack leverages the physical objects as triggers, thus making them a credible threat against deep learning systems, i.e., the trigger is ``white tape" on the forehead in the face recognition task. To achieve his goal, the adversary often manipulates the poisoning data of one or many compromised clients. However, the method to manipulate the poisoned training data that the adversary leverages vary significantly and could be roughly classified into three main approaches as follows.

% \begin{enumerate}[1)]
\noindent\textbf{Label-flipping attack. }
In \cite{fung2018mitigating,SemiTargetedMP-Sun2022,tolpegin2020data}, the adversary's poisoning strategy is directly flipping the label of the benign samples belonging to compromised clients into their targeted ones. For instance, the all images of class ``1" are labeled as ``0" in~\cite{fung2018mitigating} and images of ``dog" are flipped to ``cat" in~\cite{tolpegin2020data}. On the other hand, in ~\cite{bagdasaryan2020backdoor}, the attacker only targets the set of samples with specific features lying in the originality of the samples. These features may be the unusual car color (e.g., green), the presence of a special object in the scene (e.g., stripped pattern), or a trigger sentence ending with an attacker-chosen target word in a word prediction problem. ~\cite{Nguyen2020PoisoningIoT} proposed an attack scenario to backdoor FL-based IoT Intrusion Detection System, in which the adversary targets that packet sequences of malicious traffic from specific malware (e.g., IoT malware like Mirai malware) are not detected as malicious traffic. To achieve this purpose, the adversary moderately inserts malicious network traffic patterns into the training set including benign traffic data. The key common underlying these techniques is that the targeted set of samples contains specific characteristics, belongs to the same raw class, and these samples may be likely to appear in the training set of benign clients. 

\noindent\textbf{Out-of-distribution attack. }
In the label-flipping attack method mentioned above, the effect of the backdoor may be diluted since other benign clients contain a clean sample from the targeted class~\cite{Gong2022-survey}. Therefore,~\cite{wang2020attack,rare-Yoo2022BackdoorAI} employ the samples far from the global distribution and not likely to appear on the validation set of the training set of benign clients to backdoor the model. Specifically, the author in~\cite{wang2020attack} proposed an edge-case backdoor attack, in which the adversary targeted the edge-case samples (e.g., Southwest airplane images), which are not likely to appear in the benign clients' training data, that is, they are located in the tail of the input distribution (e.g., CIFAR-10~\cite{CIFAR-10}). Besides, authors in~\cite{rare-Yoo2022BackdoorAI} proposed ultimate rare word embedding to trigger the backdoor in Natural Language Processing domain. The rationale behind it is that rare words do not occur in the train or test sets of the clean sample by definition, which means it has little to no effect on learning the main task while it sufficiently influences the model output when present in the input. The main difference between this approach and the previous one is that the targeted set samples often lie in the tail of data distribution of the benign clients so that the impact of the backdoor will not be easily diluted. 

\noindent\textbf{Noise-instance attack. }Different from the two mentioned above approaches,~\citep{PoisonGAN} proposed to train a GAN network during the local training process and employ the shared model to generate crafted samples and leverage these samples to backdoor the model. Since the adversary may be not known about the data distribution of benign clients, so leveraging the GAN network to mimic other participants’ training samples helps the attack conduct a stealthier backdoor attack~\citep{PoisonGAN}. In recent years, the idea of employing GAN to generate these poisoned samples has become popular ~\citep{zhang2019poisoning,Zhao2022CLPACP}, and it opens a new potential direction to conduct backdoor attacks in FL.
% \end{enumerate}

\subsubsection{Artificial backdoor. }In this strategy, the ``trigger key" does not naturally exist in the samples, but is often intentionally inserted during the training process. Therefore, the targeted set of samples that the adversary tries to lead the model to misclassify is the set of samples associated with one or more backdoor patterns. The key idea of this strategy of attack is to poison a model such that in the presence of a backdoor trigger (e.g., a small square in the image), the model will misbehave while maintaining normal behaviors in the absence of a trigger. This strategy of attack is similar to a "digital attack" in ML, in which the adversary digitally inserts a random pixel block into an input~\citep{Wenger2021PhysicalBA}. To achieve his goal, at the data preparing procedure, the adversary manipulates the poisoned training data of compromised clients by injecting trigger pattern(s) to clean images and flipping the corresponding labels to the targeted one, then attackers submit their updates to the server for model aggregating. In the inference stage, the attackers use the predetermined trigger pattern(s) to trigger the learned model to perform abnormally. Based on the homogeneous property of the trigger inserted, we can roughly classify it into three main approaches as follows.

% \begin{enumerate}[1)]
    \noindent\textbf{Single-trigger attack. }
    Existing backdoor attacks against FL are mainly based on a single backdoor trigger, that is, all the compromised clients inject the same trigger into their local training dataset~\citep{Gu2019BadNetsEB,bagdasaryan2020backdoor,Sun2019CanYR,Liu2021BatchLI-VFL}. The trigger used in this approach is often set randomly and determinedly (e.g., square, cross patterns at the redundant pixels of images). At the inference process, the inserted trigger(s) to malicious clients are employed to trigger the aggregated model. Although the effectiveness of the backdoor inserted is proved to be significant~\citep{bagdasaryan2020backdoor}, the above works have not fully exploited the decentralized nature of the FL as they embedded the same trigger(s) to all adversarial parties~\citep{Xie2020DBADB}.
    
    \noindent\textbf{Distributed-trigger attack. }
    Observing the shortage of the previous approach,~\cite{Xie2020DBADB} decomposed the objective trigger into multiple local triggers and insert them into the corresponding compromised parties. This kind of attack was named a Distributed backdoor attack (DBA) and proved to be more effective than the single-trigger attack mentioned above. Specifically, each adversarial party uses the training data poisoned with its local trigger and sends the poisoned update to the server after completing local training. Unlike the previous approach, rather than directly using the local triggers independently, the adversary uses them to form a global trigger to trigger the model. Interestingly, even though the global model has not appeared during the training process, DBA could achieve a higher attack success rate and remain stealthier than the single-trigger attack strategy. 
    
    \noindent\textbf{Coordinated-trigger attack. }
    As observed from the two previous approaches, the trigger selected by the adversary is often generated independently from the learning model and not associated with the learning process (e.g., a logo, a sticker, or a pixel perturbation). Therefore, such single-trigger backdoor attacks do not fully exploit the collaboration among multiple malicious users during the training process~\citep{Gong2022CoordinatedBA}. To address this shortage,~\cite{Gong2022CoordinatedBA} newly introduced model-dependent trigger to inject the backdoor more efficiently. The model-dependent trigger is generated by seeking the optimal value assignment of the trigger (shape, size, and placement) through a sub-training process with the objective is minimizing the difference between the activation value with the expected one of a chosen neuron. After the local trigger is generated by the adversarial party, the local training dataset will be poisoned based on the trigger. At the inference step, the global trigger is constructed by the combination of local triggers, this idea is analogous to~\citep{Xie2020DBADB}. To this end, the model-dependent trigger is proven to be more efficient than the standard random trigger in previous works.
    
% \end{enumerate}

\subsection{Model Poisoning}
In FL, even after successfully inserting the backdoor into the aggregated model, the impact of the backdoor is diluted due to the aggregation process involving many benign updates~\cite{bagdasaryan2020backdoor,Neurotoxin,Gong2022CoordinatedBA}. As a result, to boost the effect of the backdoor attacks, many works were proposed to poison the model before submitting the local updates for aggregation. This strategy requires that the adversary has complete control over the training procedure and the hyperparameters (e.g., number of epochs and learning rate) and is free to modify the model parameters before submitting~\cite{bagdasaryan2020backdoor}. This technique demonstrates its efficiency when combined with data poisoning attacks in various scenarios in the literature~\cite{bagdasaryan2020backdoor,wang2020attack,Liu2021BatchLI-VFL,rare-Yoo2022BackdoorAI}. Based on the range of poisoned parts in model parameters, we can categorize existing works into \textit{Fully poisoning attack} and \textit{Partially poisoning attack} as followings.\\

\subsection{Fully poisoning attack. }
Since the most common way of aggregating the local updates from clients is the average method, the most naive way to strengthen the effect of backdoors is scaling the updates from adversarial clients to dominate the updates from the benign ones. Therefore, most of the state-of-the-art model poisoning attacks mainly utilize a hyperparameter to scale up the effectiveness of the client’s malicious mode. Moreover, the malicious models submitted are often fully poisoned by training procedures on poisoning data before scaling. 
% \begin{enumerate}[i]
    % \item \textbf{Naive approach}:\\
    \citep{bagdasaryan2020backdoor} first introduced the Model replacement method, in which the attacker ambitiously attempts to substitute the new global model with the poisoned model by scaling the poisoned update by a wisely-chosen factor. This technique requires careful estimation of global parameters and is effective when the global model is close to convergence ~\citep{bagdasaryan2020backdoor}. This technique is widely used in later works and demonstrates its success in intensifying the backdoor~\citep{Sun2019CanYR,wang2020attack}. However, directly scaling seems to be naive to be successful due to the variety of FL defenses in the literature, and the robustness of FL is more seriously considered. 
    % \item \textbf{Stealthy approach}:\\
    % since along with the advances in backdoor attack strategies, many defenses were brought to detect the anomalies among the updates, which raises a need for more stealthier model poisoning attack strategies. 
    This raises a need for stealthier model poisoning attack strategies, and as a result, many efforts were taken to address this necessity.\\
    % \begin{enumerate}[1)]
        \textbf{Constraint-based. }In this approach, the adversary constraints the local updates from the malicious clients such that they are not identified by the anomaly detector at the server by making assumptions by feasible anomaly detectors might be employed.~\citep{bagdasaryan2020backdoor,Bhagoji2019AnalyzingFL} proposed to modify the objective (loss) function by adding anomaly detection terms. The terms considered are formulated from the assumptions of any type of anomaly detection (e.g., the p-norm distance between weight matrices, validation accuracy). In~\citep{Sun2019CanYR,wang2020attack}, PGD (projected gradient descent) attack is introduced to be more resistant to many defense mechanisms. In a PGD attack, the attacker periodically projects their model on a small ball, centered around the global model of the previous iteration so that at every FL round the attacker’s model does not deviate significantly from the global model. Along with the line,~\citep{ALittleIsEnough2019} established a method to calculate a perturbation range in which the attacker can change the parameters without being detected even in i.i.d. settings. From this perturbation range, an additional clipping step is conducted to better cover the malicious updates. \\
        \textbf{Information-leakage based.} More recently,~\citep{Liu2022TechnicalRA} reported that an early-injected single-shot backdoor attack is ineffective, so they introduced a novel information leakage-assisted two-phase FL backdoor attack to strengthen the early-inserted backdoor attack. In specific, the adversary generates a crafted auxiliary dataset by leveraging information leakage about global data distribution and conducts training on this auxiliary dataset to facilitate the convergence of the FL model. The rationale behind it is that training on the auxiliary dataset whose distribution aligned with the inferred whole population distribution can facilitate the convergence of the FL model and reduce the magnitude of local model updates from normal clients, and further boost the performance of the backdoor attack.\\
        \textbf{Gradient-replacement based.} The model poisoning attack strategies mentioned above originate from the design of Horizontal FL, wherein the participating parties own the labels of their data training samples. However, to the best of our knowledge, these techniques have not been verified or fully investigated in the Vertical FL scheme. Due to this fact,~\citep{Liu2020BackdoorAA,Liu2021BatchLI-VFL} introduced Gradient-replacement backdoor attack, which is applicable to VFL even when the adversary owns only one clean sample belonging to the targeted class. Specifically, the attacker in~\citep{Liu2020BackdoorAA} records the intermediate gradients of clean samples of the targeted class and replaces the gradients of poisoned samples with these ones and uses these poisoned gradients to update the model.~\citep{Zou2022VFL} shown that even with HE-protected communication, the backdoor attack can also be conducted by directly replacing encrypted communicated messages without decryption using gradient replacement method. 
    % \end{enumerate}
% \end{enumerate}

\subsection{Partially poisoning attack. }
Different from the previous direction, which is fully poisoning the model parameters of the malicious clients,~\citep{Zhou2021DeepMP} demonstrated that the backdoor insertion could be conducted effectively without fully poisoning the whole space of model parameters. Specifically, they proposed an optimization-based model poisoning attack that injects adversarial neurons in the redundant space of a neural network to keep the stealth and persistence of an attack. To determine the redundant space, the Hessian matrix is leveraged to measure the distance and direction (i.e., “important”) of the update for the main task for each neuron. Then, an additional term is added to the loss function to avoid injecting poisoning neurons in positions that are particularly relevant to the main task. More recently,~\citep{Neurotoxin} proposed a Neurotoxin attack, wherein the adversary employs the coordinates that the benign agents are unlikely
to update to implant the backdoored model to prolong the durability of the backdoor. In Neurotoxin, instead of directly updating the poisoned model by gradient computed on poisoning data, the attacker projects gradient onto coordinatewise constraint, that is the bottom$-k\%$ coordinates of
the observed benign gradient. The common objective of partially poisoning attacks is to prevent catastrophic forgetting of the adversarial task and prolong the durability of the backdoor's impact. 
% \textcolor{orange}{constraint, assumption, similarity of all attacks strategies}
% \subsection{Metric for Attack Strategies}
% Since the objective of the adversary when trying to implant a backdoor into the model is to mislead the global model to mis-classify all the backdoored inputs (i.e., images
% with backdoor trigger) into the targeted false label while maintaining normal behaviors on the normal inputs. Therefore, the matrices to measure the efficiency of a backdoor attack are necessarily associated with the objective of the backdoor attack. 
% The first metric, named attack success rate (ASR), which measures the effectiveness of backdoor attacks, computed as
% the percentage of malicious inputs that are mis-classified to the targeted label by the backdoor. Other terms such as backdoor task accuracy ~\citep{wang2020attack}, poisoning accuracy ~\citep{?} refers to the same meaning as ASR. \\
% Mathematically, let $\tilde{\mathbf{\mathcal{D}}}$ be the targeted samples (e.g., images inserted trigger pattern), and the $\tau$ be the targeted class of the adversary. Since the backdoored model $\mathbf{f}_{\textbf{W}}$ is expected to misclassify $\tilde{\mathbf{\mathcal{D}}}$ as $\tau$, the ASR is calculated by:
% \begin{equation}
%     \text{ASR} = \sum_{x\in \tilde{\mathbf{\mathcal{D}}}} \frac{ \mathbf{f}_{\mathbf{W}}(x) = \tau}{| \tilde{\mathbf{\mathcal{D}}} |}
% \end{equation}
% In the meantime, the trained model $\mathbf{f}_{\textbf{W}}$ needs to behave normally on the benign samples (e.g., other images without the trigger). Let denote $\mathbf{\mathcal{D}} := \left[ x_1^{y_1}, x_2^{y_2}, \dots,  x_{|\mathbf{\mathcal{D}}|}^{y_{|\mathbf{\mathcal{D}}|}}\right]$ as the validation set that the the aggregator may hold, then the MTA is expressed as:
% \begin{equation}
%     \text{MTA} = \sum_{x_i\in \mathbf{\mathcal{D}}} \frac{ \mathbf{f}_{\mathbf{W}}(x_i) = y_i}{| \mathbf{\mathcal{D}} |},
% \end{equation}
% where $y_i$ is the corresponding label for sample $x_i$. In most of backdoor attack strategies, the adversary conducts implanting backdoor attack successfully if and only the trained model has high MTA and significant ASR~\citep{bagdasaryan2020backdoor,wang2020attack}. The simple illustration for the two common metrics are presented in Fig.~\ref{fig:backdoor-metrics}.
% \begin{figure}[hbt!]
% 	\centering\includegraphics[width=0.55\textwidth]{figures/backdoor_metrics.pdf} % Reduce the figure size so that it is slightly narrower than the column.
% % 	\vspace{-0.8em}
% 	\caption{Common metrics for backdoor attacks and defenses.}
% 	\label{fig:backdoor-metrics}
% % 	\vspace{-1em}
% \end{figure}
% % \begin{itemize}
% %     \item Attack success rate (ASR), probability that a backdoored sample is misclassified to the target label.
% %     \item Main task accuracy (MTA), evaluates the prediction accuracy of the backdoored model on benign samples.
% % \end{itemize}
% \subsection{Attack in Horizontal Federated Learning}
% \input{tables/backdoor-attack-proposals}
% \input{tables/backdoor-attack-dimension}
% \begin{figure}[hbt!]
% 	\centering\includegraphics[width=0.5\textwidth]{figures/hfl-pipeline.pdf} % Reduce the figure size so that it is slightly narrower than the column.
% % 	\vspace{-0.8em}
% 	\caption{General threat model of backdoor attack on HFL.}
% 	\label{fig:backdoor-hfl}
% % 	\vspace{-1em}
% \end{figure}
% \noindent\textbf{Common threat model. }Since the backdoor attack is often associated with a specific target class, it's more straightforward for the adversary to poison its training data if the adversary holds the labels for their samples. As a result, conducting backdoor attack on HFL is the most attractive field in FL which catches a great deal of attentions from researchers. 
% In most of existing works~\citep{bagdasaryan2020backdoor,wang2020attack,Xie2020DBADB}, the threat model is often assumed as followings:
% \begin{enumerate}[1)]
%     \item Federated training protocol: Most existing works consider the scenario there is that the aggregation server $\mathcal{S}$ is honest and there are one to several malicious clients $\mathcal{M}$, which are totally controlled by attackers $\mathcal{A}$. At each communication round, the server and participants only communicate the model updates and the server cannot inspect the training data stored on the clients. This fact makes the adversarial attacks to the federated model become one of the most significant challenges in FL.
%     \item Objective of the attacker: The adversary often aims at distorting the behaviour of aggregated model on selected input samples, i.e., $\mathcal{T}_{\mathcal{A}}$. Unlike the previous work,~\citep{lai2022model} newly introduce \textit{model transferring attack} (HNTROJ) against HyperNetFL, in which the adversary’s goal is to implant backdoors in all local models.
%     \item Assumption of attacker's capability: The adversary $\mathcal{A}$ have complete control over a set of compromised clients $\mathcal{M}$ to manipulate crafted model updates to poison the global model. To achieve his goal, the adversary is assumed to have ability to manipulate the training data as well as control training procedure of clients in $\mathcal{M}$. The larger the compromised set is, the higher attack success rate the the adversary could achieve. 
%     \item Common backdoor attack strategy: To implant the backdoor into the aggregated model effectively, the adversary first (1) manipulates the poisoned training data of clients in $\mathcal{M}$, then (2) poisons the local model parameters during and after training procedure and finally, (3) scales the local updates wisely to avoid being detected and better poison the aggregated model. 
% \end{enumerate}
% \textbf{Comprehensive Comparison. }We first compare the existing attacks in the following eight dimensions in Table~\ref{tab:backdoor-attack-comparision}. Then, we explain in detail each dimension considered to compare in Table~\ref{tab:attack-dimension}.

% \noindent\textit{Backdoor Characteristics. } \\
% Most of state-of-the-art attacks follow the common attack strategy which combines data poisoning and model poisoning to intensify the backdoor effect. For example, as reported in~\citep{Xie2020DBADB}, the distributed backdoor attack without scaling achieve low attack success rate (i.e., below 5\%); meanwhile, using scale factor wisely can boost the ASR to approximately 100\%. Other attack with solely data poisoning requires the continuous attack to achieve successfully backdoor effect (i.e., the malicious partipants are selected in multiple rounds). For instance, in~\cite{wang2020attack}, with the assumption that one malicious client can join the FL training every 10 rounds, the adversary can achieve almost 80\% of backdoor task accuracy in digit classification on EMNIST. The attack which requires only data poisoning is easy to conduct for even non-tech adversary with limited capability and knowledge about the training protocol as well as aggregation operator.

% \noindent\textit{Adversary Capability. }\\
% In addition to the adversary's in common threat model, authors in~\citep{PoisonGAN,SemiTargetedMP-Sun2022,Liu2022TechnicalRA} proposed using customized local training mechanism instead of simply varying number of local epochs or training parameters, i.e., training additional GAN network to generate poisoning samples in alignment with the data population of the benign clients \citep{PoisonGAN}.\\
% To conduct effective backdoor attack, the participant collusion is employed. The higher colluding ratio, the stronger attack (cf.~\citep{Sun2019CanYR}). As a result, the backdoor durability is also increased when the adversary owns large number of compromised clients. However, the malicious clients often account for just a small portion among total clients in practical scenario, i.e., $\left[0.01, 1\right]\%$ (cf.~\citep{Shejwalkar2021BackTT}). Therefore, the assumption about the large ratio of malicious participants may not be hold. In most of the proposed attacks~\citep{fung2018mitigating,wang2020attack,Xie2020DBADB,Nguyen2020PoisoningIoT}, the malicious clients are assumed to participate in multiple training rounds, i.e., continuous attack. However, this kind of attack may not be hold practically since the number of participants randomly selected in each training round is much more smaller than total clients, which means the probability that an adequate ratio of $\mathcal{M}$ joining training is very small. The direct solution for this is an effective single-shot attack~\citep{bagdasaryan2020backdoor,Liu2022TechnicalRA}. This approach seems practical since each malicious client may be selected only once in the large-scale FL system (cf.~\citep{Shejwalkar2021BackTT}).

% \noindent\textit{Attack efficiency. } \\
% % \textit{Model Poisoning Necessity. }\\
% % \textit{Highest Accessibility. }\\
% % \textit{Participant Collusion. }\\
% % \textit{Attack Frequency. }\\
% % \textit{Training Stage Constraint. }\\
% % \textbf{Backdoor attack issues. }\\
% % \textbf{Backdoor durability. }
% The efficiency of an attack is evaluated under three key dimensions: stealthiness, durability and flexibility. \\
% \noindent One of the biggest challenges to backdoor attack designing is that the malicious clients often account for just a small portion among total clients in reality, i.e., $\left[0.01, 1\right]\%$ (cf.~\citep{Shejwalkar2021BackTT}). Therefore, the poisoned updates may be easily diluted by the benign updates. This phenomenon is also known as ``catastrophic forget" in machine learning. The techniques aim to replace the global model with the poisoned one~\citep{bagdasaryan2020backdoor} or continuously remind the global model about the backdoor task by continuous participation of malicious clients~\citep{Xie2020DBADB} can prolong the backdoor effect. Another approach tried to implant backdoor into the neurons which are least overlapped with the active neurons for the main task by employing the rare samples~\citep{rare-Yoo2022BackdoorAI,wang2020attack}. More recently, the durability of the backdoor is more seriously taken into account in~\citep{Neurotoxin,Liu2022TechnicalRA,Zhou2021DeepMP} and this opens a new novelty to design a robust and durable backdoor attack. \\
% \noindent Conspicuous backdoor attack is hard to be practical since the various defenses available for aggregation server. It is trivial that the scaled malicious updates may have abnormally large values compared to the benign ones, which may easily detected.
% % by the defender at the aggregation server. Therefore, even the straight-forward defense mechanisms (i.e., smoothness and perturbation proposed by ~\cite{xie2021crfl}) could reduce the backdoor effect of scaling-based model poisoning attack. 
% Realizing this fact, many approaches consider utilizing additional techniques together with scaling the poisoned updates to make the backdoor more resistant against a range of defense mechanisms (i.e., PGD attack~\citep{Sun2019CanYR}, constrain-and-scale~\citep{wang2020attack}). However, whether these techniques are robust against state-of-the-art defense mechanisms is still an open question. \\
% The flexibility of a backdoor attack strategy is an important factor to be considered in real-world scenario. Therefore, an attack should not depend on many constraints such as training stage (i.e., early training rounds or converged training rounds), number of malicious participants, etc.
% % or investigating the redundant neurons w.r.t the main task~\citep{}
% % Although the proposed backdoor attacks in Table~\ref{tab:backdoor-attack-comparision} is proved to be efficient in specific scenarios, there are existing following significant limitations: \\
% % One of the biggest challenges to backdoor attack designing is that the malicious clients often account for just a small portion among total clients in reality, i.e., $\left[0.01, 1\right]\%$ (cf.~\citep{Shejwalkar2021BackTT}). Therefore, the poisoned updates may be easily diluted by the benign updates. To deal with this issue, the malicious clients are assumed to participate in multiple training rounds (i.e., continuous attack) as discussed in~\citep{fung2018mitigating,wang2020attack,Xie2020DBADB}. However, this kind of attack may not be hold practically since the number of participants randomly selected in each training round is much more smaller than total clients, which means the probability that an adequate ratio of $\mathcal{M}$ joining training is very small. As a result, attack strategies to intensify the backdoor effect on global model once the poisoned updates are aggregated are proposed.\\
% % The direct solution for this is an effective single-shot attack~\citep{bagdasaryan2020backdoor,Liu2022TechnicalRA}. This approach seems practical since each malicious client may be selected only once in the large-scale FL system (cf.~\citep{?}). However, the stage that the backdoor is implant directly influences the efficiency and duration of the backdoor. Specifically, the model replacement method demonstrate its proficiency when the global model is close to convergence~\citep{bagdasaryan2020backdoor}. As observed from~\citet{Xie2020DBADB}, the backdoor conducted at the initial round is gradually diminished by the benign updates. Hence, whether model replacement attack is effective if it is implanted at the early stage or the model convergence status is incorrectly estimated is still an open question. \\

% % \textit{Conspicuous backdoor attack. }The main concern related to the above-mentioned strategies is the stealthiness of the attack. It is trivial that the scaled malicious updates may have abnormally large values compared to the benign ones, which may easily detected by the defender at the aggregation server. Therefore, even the straight-forward defense mechanisms (i.e., smoothness and perturbation proposed by ~\cite{xie2021crfl}) could reduce the backdoor effect of scaling-based model poisoning attack. Realizing this fact, many approaches consider utilizing additional techniques together with scaling the poisoned updates to make the backdoor more resistant against a range of defense mechanisms(i.e., PGD attack~\citep{Sun2019CanYR}, constrain-and-scale~\citep{wang2020attack}). However, whether these techniques are robust against state-of-the-art defense mechanisms is still an open question. \\

% % \textit{Backdoor attacks with limited knowledge about data population. }Existing
% % backdoor attacks typically require clean samples to implant new backdoors~\citep{wang2020attack}. Moreover, to preserve the performance of poisoned model updates on the main task, the adversary needs to collect enough data from whole population's data distribution\textcolor{red}{cite}. However, this fact may not be facilitated practically and more often, the adversary only has access to a pre-trained model but no training set. Unlike the common approach, authors in~\citep{PoisonGAN,Liu2022TechnicalRA} do not assume about the amount of clean data that the adversary has is large, they proposed to mimic the whole population training data to boost the efficiency of backdoor attack (i.e., by using GAN\textcolor{red}{cite} or mathematical estimation). This problem should be seriously considered when designing backdoor attack in Federated Learning. 

% % When the adversary only has
% % access to a pre-trained model but no training set, attacks
% % are often only able to extract backdoors from a model,
% % rather than inducing a vulnerability to a desired trigger

% % For example, 
% % such as Projected Gradient Descent~\citep{Sun2019CanYR}, \\
% % \textbf{Small number of compromised clients. }\\
% % \textbf{Limited adversary capabilities. }\\
% % \textbf{Unpractical backdoor attack. }\\
% % - What's the challenges for current backdoor attacks in HFL (dilution, not many chance to participate, no knowledge about the data distribution of the benign clients ==> easy to detect, the availability of current defense ==> a need for more stealthy attack?, sth related to the fairness and contribution (need to survey, some assumption may not hold.) \\
% % - More recently, more efforts are made to prolong the impact of the backdoor (Why? - the assumption about continuous attack may be difficult to be practical on some scenarios (cite if possible) => the effort to make the backdoor more durable is very necessary). For example, if a participant only can involve in to very few or even only 1 round (=> e.g., very large-scale FL system). \\
% % - Colluding attacks: (may be possible), its effect is proved through the intensive experiments ==> dangerous and really need to be careful. 
% % - To prevent dilution from the updates of benign clients


% % \textcolor{blue}{
% % \begin{itemize}
% %     \item A basic attacking pipeline (with figure)
% %     \item Most of backdoor attacks make assumptions: honest server, the adversary controls one to several clients in the FL system.
% % \end{itemize}
% % }
% % \subsubsection{Discussion}
% \subsection{Attack in Vertical Federated Learning}
% \begin{figure}[tbh]
%      \centering
%      \includegraphics[width=0.6\textwidth]{figures/backdoor-vfl.pdf}
%      \caption{\textbf{A common backdoor attack scheme in Vertical FL.}}
%      \label{fig:vfl_attack_pipeline}
%  \end{figure}
% Due to the difference in the mechanism between Horizontal FL and Vertical FL, the attack strategy is varied. The following attack scheme is considered:  (i) the attacker has access to the training data of one or more data parties $D_m$ and it controls the training procedure and local hyperparameters of attacked parties. (ii) The attacker can modify local updates such as training weight and gradients before sending transmitted data to other parties. (iii) The attacker does not control any benign parties’ training nor does the attacker control the global communication and aggregation protocols. (iv) Contrary to traditional data poisoning attacks which focus on poisoning training data, the attacker in collaborative learning focus on poisoning gradients and model updates that are communicated among parties in the protocol.
% The main difference between backdoor attacks on Horizontal FL and Vertical FL is that: in VFL, the attacker only has access to a portion of the feature space of parties that it controls, and it may not have access to labels if it doesn’t control the active party. Moreover, it also has only a portion of the model parameters of the parties it controls.\\

% VFL is under-studied for the lack of datasets and benchmarks~\citep{Cai2022AcceleratingVF}, so there are not so much effort put for the backdoor attack on VFL. To the best of our knowledge,~\cite{Liu2021BatchLI-VFL} first introduced \textit{Gradient-replacement backdoor} by wisely swap the gradients of benign and poisoned samples before sending back to the active party. This method is proved to be effective in the later work~\citep{Zou2022VFL} even when the communication between parties in FL is protected by Homomorphic encryption (HE)~\citep{HE2020}.
% % \begin{itemize}
% %     \item A basic attacking pipeline (with figure)
% %     \item State-of-the-art Attack strategies
% % \end{itemize}

% % \subsection{Discussion}
% % \begin{itemize}
% %     \item Realistic backdoor attack scenarios. 
% %     \item When is the backdoor effective in FL? 
% %     \item Backdoor attack in Vertical FL.
% %     \item Backdoor attack in Federated Transfer Learning.
% %     \item Backdoor attack in Hierarchical FL.
% % \end{itemize}
% % \textcolor{orange}{ Link to section 6}

% % \subsection{Open Problems}
% % \begin{itemize}
% %     \item \textcolor{red}{To the best of our knowledge, there has not been much effort taken on backdoor attack in Federated Transfer Learning, \ldots}
% %     \item \textcolor{red}{Backdoor attack in hierarchical FL is also intriguing and it opens a new direction for the researcher to find the potential vulnerabilities in this scheme, \ldots}
% % \end{itemize}


==> intro-2023.tex <==
\subsection{Federated Learning}
Together with the development of the digital century is the generation of a huge amount of data in various fields, and a great deal of efforts is taken to employ this valuable data. However, this data is often distributed across different devices and may contain highly confidential or sensitive information, which is not easy to publicly access. This fact challenges the centralized training, i.e., collecting data and training on a centralized  \textcolor{purple}{repository} due to privacy \textcolor{purple}{concerns}. Motivated by this challenge, Federated learning (FL)~\citep{McMahan2016FederatedLO,Bonawitz2019TowardsFL} emerges as a collaborative training method to leverage the variety of data without compromising its privacy. In FL, \textcolor{purple}{unclear} data are stored on end-user devices, which cooperate together to train a global model. On an orchestration server, only locally computed updates and analysis results are collected and aggregated to update the global model. The updated model is then distributed to end-users to facilitate knowledge sharing. The variety of the end-user devices make FL efficient in various fields such as natural language processing (NLP)~\citep{Chen2019FederatedLO,Lin2021FedNLPAR}, healthcare~\citep{Xu2021FederatedLF,Prayitno2021ASR,Gupta2021HierarchicalFL,Liu2021FederatedLA}, internet of things (IoT)~\citep{Liu2021DeepAD,Kholod2021OpenSourceFL,Nguyen2021EfficientFL}. \textcolor{purple}{Privacy and security is widely studied in FL~\cite{Abdulrahman2021ASO,Yin2021ACS,Mothukuri2021ASO,Gosselin2022PrivacyAS}. Nevertheless, despite being more privacy friendly than the centralized approach, FL is still subject to attacks that may lead to the learned model’s misbehavior. A typical example is adversarial attacks, which aim to distort the model by sending poisoned local model. Since the orchestration server cannot directly verify the data, the centralized federated learning architecture facilitates this type of attack.}\\

\textcolor{purple}{There are two types of adversarial attacks that can be launched against machine learning models during the training phase: targeted and untargeted attacks.
In untargeted attacks~\cite{blanchard2017machine,bernstein2018signsgd}, the attacker attempts to cause the classifier to produce incorrect results, i.e., causing the model to converge to a sub-optimal local minima or diverge completely. For instance, adversarial attacks  aim to misclassify a handwritten ``7" as any other number. These attacks, also known as convergence attacks, can be easily detected by analyzing the model's accuracy on validation data. On the other hand, targeted attacks~\cite{bhagoji2019analyzing, chen2017targeted, liu2017trojaning} seek to cause the model to misclassify a specific group of samples while minimizing the impact on its performance on the main task. For instance, the adversary uses a model that categorize a handwritten ``7" as a ``4". These types of attacks are also known as backdoor attacks, and they aim to deceive the backdoored model into behaving abnormally on any sample marked with a backdoor trigger~\cite{chen2017targeted, liu2017trojaning}, while behaving normally on all other samples.}
\subsection{Backdoor Attacks in FL} 
Backdoor attack is well-known term in machine learning (ML) and is studied in-depth~\citep{Chen2017TargetedBA,Salem2022DynamicBA,Goldblum2022DatasetSF}. The key idea behind this type of attack is to ``poison" a model so that a backdoor trigger in a test-time input causes the model to behave in a specific manner (assign a predetermined label) that the attacker desires. Meanwhile, to ensure stealthiness, the poisoned model should behave normally without the presence of triggers. Unlike backdoor attack in ML, in the FL setting, an adversary can insert poisons at various stages of the training pipeline, and attacks are not constrained to be ``clean-label". \textcolor{purple}{In this case, users have complete control over the training data and labels seen by their device, in addition to the content of updates sent to the orchestration server. At the same time, federated learning adversaries are weak and their impact on the entire training system is limited by the contribution from many other users. As a result, the adversaries need to customize their attack strategies by employing the FL's specialized features to strengthen their attacks. This is the reason leading to the variety of backdoor attack strategies in FL as well as the corresponding defenses.}
% ~\textcolor{purple}{Need more statement about the differences between backdoor attack in ML and FL?} 
% This is the reason leading to various threats to FL and turning it into an attractive land for backdoor attacks. 
Indeed, much effort was devoted to demonstrates that FL is vulnerable to the backdoor attack and with a carefully-designed attack scheme, the adversary can successfully manipulate the global model without being detected~\citep{bagdasaryan2020backdoor,wang2020attack,Xie2020DBADB,Neurotoxin}. Backdoor attack in FL has developed over time with enhancements in the effectiveness and stealthiness, which motivated us to write this survey. It is worth noting that most of the existing attacks focus on Centralized FL (cf. Fig.~\ref{fig:fl-centralized}), in which the orchestration server is assumed to be honest and there may be \textbf{one to many }malicious participants who try to manipulate poisoned updates. The attack strategies can be discriminated in term of multiple dimensions such as: attack training phase, attack target, attack manner, etc. Specifically, the adversary can conduct attacks at many stages of the training pipeline (i.e., data poisoning and model poisoning) with different assumptions about adversary capability. Even with limited accessibility, the adversary can leverage the advances in ML (i.e., GAN, posterior probability) to obtain the necessary knowledge so as to conduct a successful attack~\citep{PoisonGAN,Liu2022TechnicalRA}. The combination of existing methods (i.e., edge-case combined with a projected gradient attack proposed in~\cite{wang2020attack}) makes the attack stronger and stealthier. Different from centralized training, a backdoor attack in FL is easily diluted by the benign updates from non-adversarial participants, but many newly introduced techniques have been proposed to prolong the durability of the backdoor ~\citep{Neurotoxin,Zhou2021DeepMP,Liu2022TechnicalRA}.\\



% CE-Fed: Communication efficient multi-party computation enabled FL
% \begin{figure}[hbt!]
% 	\centering
% 	\includegraphics[width=0.65\textwidth]{figures/centralized_fl.pdf}
% % 	\vspace{-0.8em}
% \caption{Centralized Federated Learning. }
% % 	\href{https://www.sciencedirect.com/science/article/pii/S2590005622000546}{Source} }
% 	\label{fig:fl-centralized}
% 	% \vspace{-1em}
% \end{figure}

\begin{figure}[hbt!]
	\centering
	\includegraphics[width=0.55\textwidth]{figures/FL-BA-overview.pdf}
% 	\vspace{-0.8em}
\caption{Overview of Backdoor Attacks and Countermeasures in FL.}
% 	\href{https://www.sciencedirect.com/science/article/pii/S2590005622000546}{Source} }
	\label{fig:overview}
	% \vspace{-1em}
\end{figure}
% \textcolor{red}{Adding a figure about Decentralized Federated Learning}
\subsection{Defenses against the Backdoor Attack}
Due to the strength and risky consequences of backdoor attacks, many works were devoted to designing FL-robust defense mechanisms to mitigate or remove the backdoor effects, which is illustrated in Figure~\ref{fig:overview}. These techniques can be conducted in different phases of FL's learning procedure, which includes pre-aggregation, in-aggregation, and post-aggregation. Regarding each phase, the methods used share some common characteristics related to objectives and methodologies. 
Specifically, before aggregation process,~\cite{fung2018mitigating,Nguyen2022-FLAME,rieger2022deepsight,shen2016auror} proposed to determine malicious updates based on their defined similarity metrics and remove or reduce these corresponding contributions to the aggregated model. On the other hand, many proposed more robust aggregation operators and replaced the standard aggregation method so as to alleviate the backdoor effects~\citep{Pillutla2022RobustAF,Sun2019CanYR,Blanchard2017MachineLW,Ozdayi2021DefendingAB}. Unlike the previous approaches, which tried to \textcolor{purple}{prevent global from being backdoored by poisoned models},~\citep{Wu2022FederatedUL,Wu2020MitigatingBA} tried to repair the backdoored model, which is the aggregation of both benign and malicious updates. Unlike defenses in ML, in the FL scheme, the local training data can not be easily investigated \textcolor{purple}{since the training data are kept private at all clients}. Then, methods such as major voting and statistical mechanisms~\citep{Wu2020MitigatingBA,Weber2020RABPR,Yun2019CutMixRS} which require data investigation, are not applicable to FL.\\
% Backdoor attack strategies and defense mechanisms vary significantly and undergo great evolution.
\textcolor{purple}{Because attacks and countermeasures are applied differently in machine learning and federated learning, existing studies on backdoor attacks in machine learning are not perfectly applicable to federated learning.} This necessities a thorough review of existing works related to backdoors attack and defenses specialized for FL. \textcolor{purple}{To this end, we first review the related surveys and their shortages in discussing FL backdoor attacks, and then summarize our contribution.}\\
\input{tables/related-survey.tex}

\subsection{Related Surveys}
% \textbf{Related survey works.} 
There are various survey papers in the literature that discuss backdoor attack to some extend. We review the relevant works in terms of contribution summary and main focus topic in Table~\ref{tab:survey-summary}.
\textcolor{purple}{Several surveys addressing security issues in federated learning have been published in recent years and they mentioned backdoor attack as one of the biggest challenges~\cite{Abdulrahman2021ASO,Yin2021ACS,Mothukuri2021ASO,Gosselin2022PrivacyAS}. 
% Their survey introduced several distinguished poisoning attacks against FL. 
In these works, backdoor attack is viewed as a specific instance of the target poisoning attack or as a special example of robustness threat~\cite{Lyu2020ThreatsTF}. Hence, backdoor attacks and their countermeasures are examined from the perspective of a poisoning attack and a security assessment in these studies. As a result, most of these surveys studied backdoor attacks in technique-driven methodology. Their survey, however, ignores the connection between the attack strategies. Furthermore, the authors did not address the limits of existing attack and defense strategies in FL. Also, defensive federated learning approaches are not addressed in terms of efficiency against various backdoor attack schemes.}
\textcolor{purple}{Another line of surveys conducted on the backdoor attacks in deep learning and federated learning is considered as one special case~\cite{Li2022BackdoorLA,Goldblum2022-wq,Chen2017TargetedBA}. However, such broad-ranging attack scenarios or evaluating criteria in ML may not be completely applied in FL, and many specialized characteristic of backdoor attacks are unique for FL systems. For example, many popular techniques such as clean-label attacks~\cite{Goldblum2022-wq} have not presented in FL, and model poisoning attack in FL is not clearly discussed in these surveys.\\
To this end, FL backdoor attacks are only one of the threats or specific cases in related surveys, which makes them contribute less on improving the understanding of working mechanism and consequent robustness vulnerabilities in FL. Recognizing this, the authors of \cite{ba-fl-survey-2022} investigated backdoor attacks as well as cutting-edge defenses employed in FL. This study, however, is primarily technique-driven in the form of a recap version, with a lack of further analysis and demonstration of the inter-connection between backdoor attacks themselves and backdoor attacks versus defenses. Furthermore, evaluation metrics and their applicability in the physical world (i.e., physical backdoor attacks) have not been discussed. It is worth mentioning that backdoor attacks evolve in conjunction with countermeasures. Recent FL backdoor attacks are designed to be an efficient yet stealthy technique for circumventing available defenses by exploiting their weaknesses. We explain the unfavourable scenario to a lack of a thorough understanding of FL backdoor attacks and their functioning mechanism. A thorough understanding of backdoor attacks will assist academia and industry in developing more robust FL systems.}
% Authors in~\cite{Chen2017TargetedBA} firstly introduced systematically the real threats to a learning system caused by backdoor poisoning attacks, and thus highlighted the importance of further investigation and proposing defense strategies against them.
% Beside backdoor attack, other attacks such as data poisoning~\cite{Goldblum2022-wq} and adversarial learning attack~\cite{Miller2020AdversarialLT} are well studied in the literature. For example, Miller at el.~\cite{Miller2020AdversarialLT} provides a contemporary survey of adversarial learning attack including individual hackers, criminal organizations, as well as government intelligence services, which may seek to ``break" the DNN systems. This study discussed both targeted attack and indiscriminate attack, in which the former is the scenario with a predefined target class to attack and the later is attack focusing on the change in performance of DNN  without ensuring a particular target class is assigned. More recently, Goldblum et al.~\cite{Goldblum2022-wq} catalog and  systematize vulnerabilities in the dataset creation process and how the resulting data poisoning can cause servers damage/ attack in both training and testing time and the corresponding defenses in the literature. In~\cite{Li2022BackdoorLA}, the authors presented an up-to-date systematic taxonomy of backdoor attacks and defenses, and give the analysis about the relation between backdoor attacks and relevant fields
% (i.e., adversarial attacks and data poisoning). Unlike the previous works, Tian et al.~\cite{Tian2022ACS} analyzes poisoning attacks and countermeasures in multi-dimension, which are untargeted poisoning attacks, target poisoning attacks, and backdoor poisoning attacks in both centralized learning and FL scenarios. This is the first survey work which provides a unified perspective to examine security vulnerabilities in both ML and FL. In these survey works, they also discuss some dimension of backdoor attack in FL to some extend associated with the concepts and perspectives from the ML in general.
% Since the evolution of FL is more and more influential, there are a dozen of survey works conducted to study about various aspects and problems related to FL privacy and security. Backdoor attack is one of the biggest challenges to the security and privacy of FL system~\cite{Abdulrahman2021ASO,Yin2021ACS,Mothukuri2021ASO,Gosselin2022PrivacyAS}. In FL, adversarial attacks may threaten the learning model and to the integrity of the privacy of data. These threats lead to the concern about robustness and privacy of FL. The robustness of FL expresses the quality of global model under targeted/untargeted attacks, while the FL privacy is threatened by the adversarial attacks leveraging shared information in FL to investigate the sensitive information about the training data (i.e., membership inference attack, model inversion attack). In earlier research, the backdoor attack is viewed as a specific instance of the target poisoning attack; hence, it is analyzed as a special example of robustness threat~\cite{Lyu2020ThreatsTF}. Backdoor attacks and countermeasures are examined from the perspective of a poisoning attack and a security assessment in these studies.
% Consequently, the systematic taxonomy and analysis of backdoor attacks and countermeasures specialized in FL is an important piece of the puzzle that is missing.\\

% \textbf{Our contribution.} 
\subsection{Our Motivation and Main Contributions}
Although the backdoor attack in ML serves as a foundation for the backdoor attack in FL, their manifestations differ owing to the different learning architectures. In addition, despite the fact that the backdoor poisoning attack is a subcategory of the poisoning/adversarial attacks, the method to implant a backdoor into FL is significantly distinct from other poisoning attacks (e.g., byzantine attacks) due to the differences in the attacking objectives. As a result, the review specialized in backdoor attacks for FL is necessary to fill in the gap of existing survey works and this is also the motivation for us to conduct this survey. This work provides an in-depth analysis of backdoor attacks and countermeasure strategies for FL. The contribution of this work can be summarized as followings:
\begin{itemize}
    \item We present a systematic taxonomy of backdoor attacks in FL based on different perspectives on their manner and purpose of attacks. \textcolor{purple}{In addition, we illustrate the connection among attacking techniques via their common features and advancement to help readers better understand the assumptions, principles, reasons and differences among these attacking stratgies}. 
    % Moreover, we illustrate the connection among techniques used in different attack scenarios with corresponding threat models and assumptions.
    \item We present the state-of-the-art defense strategies and categorize them based on their common objectives and methodologies. In addition, a comprehensive comparison and analysis about their efficiency \textcolor{purple}{against existing backdoor attacks} and their applicability is provided.
    \item Based on the comprehensive study above, we discuss the challenges for both backdoor attacks and defenses in FL, followed by possible future works in different aspects, and demonstrate significant missing gaps that need fulfilling.
    \item To the best of our knowledge, this is the first survey to assess and analyze backdoor attacks and defenses utilizing FL-specific criteria and perspectives. With the support of this comprehensive study, researchers and practitioners may better understand the properties and limitations of each backdoor attack/defense mechanism, hence facilitating the development of more advanced methods. In addition, we believe that our survey will promote a deeper knowledge of backdoor threats and countermeasures, hence facilitating the construction of more secure FL systems.
\end{itemize}
% In addition, we present the existing defense strategies with comprehensive comparison and analysis. We not only bring the taxonomies of the existing backdoor
% attacks and defenses, but also give a detailed discussion of their pros and cons and efficiency in practical scenarios. Moreover, we discuss the challenges and possible future works in different aspects, and demonstrate significant missing gaps that need fulfilling.

% \begin{figure}[hbt!]
% 	\centering
% 	\includegraphics[width=0.5\textwidth]{figures/orgnization_of_the_paper.pdf}
% % 	\vspace{-0.8em}
% 	\caption{Organization of the paper. }
% % 	\href{https://www.sciencedirect.com/science/article/pii/S2590005622000546}{Source} }
% 	\label{fig:fl-centralized}
% 	\vspace{-1em}
% \end{figure}

\subsection{Survey Organization}
% \textcolor{red}{@tuannm}
In this survey paper, we investigate the topic of backdoor attacks in federated learning (FL). The rest of the survey paper is divided into six chapters, the contents of which are as follows:
\begin{itemize}
    \item In Chapter 2, we provide background on FL and the concept of backdoor attacks in this setting.
    \item In Chapter 3, we classify different types of backdoor attacks in FL based on their approach, either data poisoning or model poisoning. We also focus specifically on HFL, in which multiple parties contribute to a single model.
    \item In Chapter 4, we examine various methods for defending against backdoor attacks in HFL. These defenses are organized based on the stage of the FL training process at which they are applied.
    \item Chapter 5 presents evaluation metrics for evaluating the effectiveness of both attacks and defenses in FL. We also compare different attack and defense strategies and discuss the unique challenges and considerations present in the setting of VFL, where a single party trains a model on data from multiple sources.
    \item In Chapter 6, we discuss ongoing challenges and potential future research directions in the area of backdoor attacks and defenses in FL. These include the development of more realistic attack scenarios and the exploration of issues related to the design and robustness of backdoor defenses.
    \item Finally, In Chapter 7, we summarize our findings and draw conclusions about the current state of the field.
\end{itemize}












==> tables/attack-defense-assessment.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[tbh]
\scriptsize
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{@{}lp{0.15\textwidth}cccccccccc@{}}
\toprule
\multicolumn{2}{l}{\multirow{3}{*}{}}                        & \multicolumn{6}{c}{Data poisoning}                                                                                                                                                                                                                                                                                                                                                 & \multicolumn{4}{c}{Model poisoning}                                                                                                                                                                                                                                           \\ \cmidrule(l){3-8}\cmidrule(l){9-12}
\multicolumn{2}{l}{}                                         & \multicolumn{3}{c}{Semantic backdoor}                                                                                                                                                & \multicolumn{3}{c}{Artificial backdoor}                                                                                                                                                     & \multicolumn{3}{c}{Fully poisoning}                                                                                                                                                         & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Partially \\ poisoning\end{tabular}} \\
\cmidrule(l){3-5}\cmidrule(l){6-8}\cmidrule(l){9-11}

\multicolumn{2}{l}{}                                         & \begin{tabular}[c]{@{}c@{}}Label\\ flipping\end{tabular} & \begin{tabular}[c]{@{}c@{}}Out of \\ distribution\end{tabular} & \begin{tabular}[c]{@{}c@{}}Noise\\ instance\end{tabular} & \begin{tabular}[c]{@{}c@{}}Single \\ trigger\end{tabular} & \begin{tabular}[c]{@{}c@{}}Distributed \\ trigger\end{tabular} & \begin{tabular}[c]{@{}c@{}}Coordinated \\ trigger\end{tabular} & \begin{tabular}[c]{@{}c@{}}Scaling\\ based\end{tabular} & \begin{tabular}[c]{@{}c@{}}Constrain\\ based\end{tabular} & \begin{tabular}[c]{@{}c@{}}Gradient \\ replacement based\end{tabular} &                                                                                 \\ \midrule
\multirow{6}{*}{Pre-aggregation}  & FLAME 2022               & YES                                                      & YES                                                            &                                                          & YES                                                       & YES                                                            &                                                                & YES                                                     &   YES                                                        &                                                                       &                                                                                 \\
                                  & DeepSight 2022           &                                                          &     YES                                                           &  YES                                                        &                                                           &     YES                                                           &   YES                               &                                     &   YES                                                        &                                                                       &                                                                                 \\
                                %   \cmidrule(l){2-12}
                                  
                                %   & Flguard 2021             &                                                          &                                                                &                                                          &                                                           &                                                                &                                                                &                                                         &                                                           &                                                                       &                                                                                 \\
                                  & VAE 2020                 &                                                          &                                                                &                                                          & YES                                                       &                                                                &                                                                &                                                         &                                                           & YES                                                                   &                                                                                 \\
                                  & FoolsGold 2018           &      YES                                                    &                                                                &                                                          &                                                           &                                                                &                                                                &                                                         &                                                           &                                                                       &                                                                                 \\
                                  & AUROR 2016               &   YES                                                       &                                                                &                                                          &                                                           &                                                                &                                                                &                                                         &                                                           &                                                                       &                                                                                 \\\midrule
% \cmidrule \\
\multirow{8}{*}{In-aggregation}   & CRFL 2021                &                                                          &                                                                &                                                          &                                                           &                                                                &       YES                                                         &                                                         &                                                           &                                                                       &                                                                                 \\
                                  & BaFFle 2021              &                                                          &                                                                &                                                          &                                                           &                                                                &                                                                &                                                         &                                                           &                                                                       &                                                                                 \\
                                  & RLR 2021                 &                                                          &                                                                &                                                          &                                                           &                                                                &                                                                &                                                         &                                                           &                                                                       &                                                                                 \\
                                  & DP 2020                  &                                                          &                                                                &                                                          &                                                           &                                                                &                                                                &                                                         &                                                           &                                                                       &                                                                                 \\
                                  & Optimised training 2020  &                                                          &                                                                &                                                          &                                                           &                                                                &                                                                &                                                         &                                                           &                                                                       &                                                                                 \\
                                  & FL-WBC 2020              &                                                          &                                                                &                                                          &                                                           &                                                                &                                                                &                                                         &                                                           &                                                                       &                                                                                 \\
                                  & FL-Pivot Training 2020   &                                                          &                                                                &                                                          &                                                           &                                                                &                                                                &                                                         &                                                           &                                                                       &                                                                                 \\
                                  & Weak DP/ Central DP 2019 &                                                          &                                                                &                                                          &                                                           &                                                                &                                                                &                                                         &                                                           &                                                                       &                                                                                 \\\midrule
\multirow{2}{*}{Post-aggregation} & KD Unlearning 2022       &                                                          &                                                                &                                                          &                                                           &                                                                &                                                                &                                                         &                                                           &                                                                       &                                                                                 \\ 
% \cmidrule(l){2-12} 
                                  & Pruning Neurons 2020     &                                                          &                                                                &                                                          &                                                           &                                                                &                                                                &                                                         &                                                           &                                                                       &                                                                                 \\ \bottomrule
\end{tabular}}
\end{table}

==> tables/backdoor-attack-dimension.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[tbh]
\centering
\caption{The Primary Dimensions of a Backdoor Attack in FL}
\label{tab:attack-dimension}
\scriptsize
\resizebox{0.9\textwidth}{!}{\begin{tabular}{c|c|c|p{0.55\textwidth}}
\hline
Dimension                                                                                   & Attribute                                                 & Values             & Description \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Backdoor   \\      Characteristics\end{tabular}} & \multirow{2}{*}{\makecell{Attack \\vector}}                            & Data Poisoning     & The adversary is able to manipulate the poisoned data on compromised clients. The clients use this data to compute their local updates.                     \\ \cline{3-4} 
                                       &        & Model Poisoning    &   The adversary is able to break into the compromised clients and directly controls the training processes and manipulate the local updates.                     \\ \cline{2-4} 
                                                                                            & \multirow{2}{*}{\makecell{Backdoor \\key}}                         & Input-instance key &      The targeted specific samples of the backdoor task are the samples naturally containing specific characteristics.                       \\ \cline{3-4} 
                                                                                            &                                                           & Pattern key        &    The targeted specific samples of the backdoor task are the samples containing intentionally-inserted patterns.                   \\ \hline
\multirow{7}{*}{\makecell{Attacker \\Capability}}                                                        & \multirow{3}{*}{\makecell{Highest\\Accessibility}}                            & Black-box          &   The adversary has no knowledge about the target model, and is only able to replace their local data set.                   \\ \cline{3-4} 
    &  & White-box  &  The adversary is able to manipulate the training data and local model training's parameters.                   \\ \cline{3-4} 
     &                                          & Full-box   &   The adversary has full control of local training process and is able to replace training protocol.                      \\ \cline{2-4} 
                                                                                            & \multirow{2}{*}{\makecell{Participant\\Collusion}}                        & Non-colluding      &  Each adversary controls one and only one participating client.                      \\ \cline{3-4} 
                                                                                            &                                                           & Colluding          &   The adversary has full control over several participants in FL system.                \\ \cline{2-4} 
                                                                                            & \multirow{2}{*}{\makecell{Attack\\frequency}}                         & Single-shot        &  During the training process, the malicious client(s) are selected in only a single round of training.                      \\ \cline{3-4} 
                                                                                            &                                                           & Continuous         &   The backdoor attacks are carried out continuously during the training process, either by all communication rounds or a portion of them.                 \\ \hline
\multirow{6}{*}{\makecell{Attack \\Efficiency}}                                                            & \multirow{2}{*}{\makecell{Training Stage \\Constraint}}                   & Early-round        &  The backdoor is effective even when it is inserted in the early training rounds.                  \\ \cline{3-4} 
                                                                                            &                                                           & Converged-round    &  The backdoor is effective only when it is implanted when the global model is close to convergence.                   \\ \cline{2-4} 
                                                                                            & \multicolumn{1}{c|}{\multirow{2}{*}{\makecell{Backdoor \\durability}}} & Fair                    &   The durability of the backdoor is diluted significantly after the attacker stops participating.               \\ \cline{3-4} 
                                                                                            & \multicolumn{1}{l|}{}                                     &  Extended   &    The durability of the backdoor is remained after the attacker stops participating.                      \\ 
                                                                                    
                                                                                \cline{2-4} 
                                                                                            & \multicolumn{1}{c|}{\multirow{2}{*}{\makecell{Stealthiness \\consideration}}} & YES                    &   The adversary tries to avoid detection by employing additional techniques to constraint the abnormal updates from malicious clients.               \\ \cline{3-4} 
                                                                                            & \multicolumn{1}{l|}{}                                     &  NO   &    The stealthiness of the attack is not mentioned or evaluated.                      \\ 
                                                                                            \hline
\end{tabular}}
\end{table*}

==> tables/backdoor-attack-proposals-bak.tex <==
\renewcommand{\arraystretch}{1.5}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[hbt]
\caption{{Comparison of State-of-the-art Backdoor Attack Strategies in FL}}
\label{tab:backdoor-attack-comparision}
\resizebox{\textwidth}{!}{
\begin{tabular}{llccccccccc}
\hline
&  & 
\multicolumn{3}{c}{Backdoor Characteristics}     & \multicolumn{3}{c}{Attacker Capability}          & \multicolumn{3}{c}{Attack Efficiency}         \\

\cmidrule(lr){3-5} 
\cmidrule(lr){6-8} 
\cmidrule(lr){9-11}
    \multirow{1}{*}{Name}  &   
    \multirow{1}{*}{Year}  & 
    \makecell{Data \\Poisoning}  & 
    \makecell{Model \\Poisoning} & 
    \makecell{Highest \\Accessibility} & \makecell{Collusion \\Required} & \makecell{Single-shot \\Attack} & 
    \makecell{Converging Stage\\Constraint} & \makecell{Extended \\Durability} &
    \makecell{Stealthiness \\Consideration} &
    \multirow{1}{*}{\makecell{Applications}} \\ 
    \hline
RE+GE~\cite{rare-Yoo2022BackdoorAI} & 2022 & \makecell{D1} & M4 & White-box & \cmark & \xmark & \xmark & \xmark & \xmark & NLP\\
CBA~\cite{Gong2022CoordinatedBA} & 2022 & D2 & -- & Full-box & \cmark & \xmark & \xmark & \xmark & \xmark & IC                                                                \\
% ILBA~\cite{Liu2022TechnicalRA} & 2022 & \xmark & M2 & Full-box & \xmark & \cmark & \xmark & \cmark & \cmark & IC                                                                   \\
Neurotoxin~\cite{Neurotoxin} & 2022 & -- & M4 & White-box & \xmark & \xmark & \xmark & \cmark & \xmark & \makecell[c]{NLP, IC}                                                                 \\
GRA-HE~\cite{Zou2022VFL} & 2022 & D2 & M3 & Full-box & \xmark & \xmark & \xmark & \xmark & \xmark & IC                                                                          \\
DeepMP~\cite{Zhou2021DeepMP} & 2021 & -- & M4 & White-box & \xmark & \cmark & \xmark & \cmark & \cmark & IC                                                           \\
PoisonGAN~\cite{PoisonGAN} & 2021 & D1 & -- & Full-box & \cmark & \xmark & \xmark & \xmark & \xmark & IC                                                                   \\
DBA~\cite{Xie2020DBADB} & 2020 & \makecell{D2} & M1, M2 & White-box & \cmark & \cmark & \xmark & \xmark & \cmark & IC                                                                           \\
PFLIoT~\cite{Nguyen2020PoisoningIoT} & 2020 & \makecell{D1} & -- & White-box & \cmark & \xmark & \xmark & \xmark & \xmark & IoS                                                                          \\
GRA~\cite{Liu2020BackdoorAA} & 2020 & D2 & M3 & Full-box & \xmark & \xmark & \xmark & \xmark & \xmark & IC                                                                      \\
Edge-case~\cite{wang2020attack} & 2020 & \makecell{D1} & M1, M2 & White-box & \xmark & \xmark & \xmark & \xmark & \cmark & \makecell[c]{IC, NLP}                                                                     \\
AnaFL~\cite{Bhagoji2019AnalyzingFL} & 2019 & -- & M2 & White-box & \xmark & \xmark & \cmark & \xmark & \cmark & \makecell{IC, LR}                                                                    \\
ALIE~\cite{ALittleIsEnough2019} & 2019 & -- & M2 & White-box & \cmark & \xmark & \xmark & \xmark & \cmark & IC                                                                                      \\
PGD~\cite{Sun2019CanYR} & 2019 & -- & M2 & White-box & \cmark & \xmark & \xmark & \xmark & \cmark & IC                                                                         \\
\makecell[l]{Constrain-and-scale}\cite{HTBD2018} & 2018 & D1, D2 & M1, M2 & White-box & \xmark &  \cmark & \cmark & \xmark & \cmark & \makecell{IC, NWP}                               \\
\makecell[l]{Model replacement} \cite{HTBD2018} & 2018 & D1, D2 & M1 & White-box & \xmark & \cmark & \cmark & \cmark & \cmark & \makecell{IC, NWP}                                       \\
Sybils~\cite{fung2018mitigating} & 2018 & \makecell{D1} & -- & Black-box & \cmark & \xmark & \xmark & \xmark & \xmark & Classification                                                                 \\

\hline
\multicolumn{2}{l}{\cmark: YES/Applicable} &
\multicolumn{3}{l}{\xmark: NO/Not Applicable} &
\multicolumn{2}{l}{--: Not Main Focus} &
\multicolumn{2}{l}{D1: Semantic} & \multicolumn{2}{l}{D2: Artificial}    \\   
\multicolumn{2}{l}{M1: Scaling-based} & \multicolumn{3}{l}{M2: Constrain-based} & \multicolumn{2}{l}{M3: Gradient-replacement} & \multicolumn{3}{l}{M4: Partially Poisoning}   \\ 

% \multicolumn{2}{l}{S-A: Single-shot Attack } & \multicolumn{3}{l}{\xmark: Continuous Attack} &\\   

% \multicolumn{2}{l}{Er-A: Early-round Attack} & \multicolumn{3}{l}{Cr-A: Converged-round Attack} \\ 

\multicolumn{2}{l}{IC: Image Classification} & \multicolumn{3}{l}{NLP: Natural Language Processing} & \multicolumn{2}{l}{LR: Logistic Regression} & \multicolumn{2}{l}{IoS: IoT System} & \multicolumn{2}{l}{NWP: Next Word Prediction}  
\end{tabular}
% \smallskip
% S: Input-instance-key, A: Pattern-key
}
\end{table*}

==> tables/backdoor-defense-proposals.tex <==
\begin{table*}[hbt!]
\scriptsize
\centering
\caption{Comparison of the State-of-the-art Defenses against Backdoor Attacks in FL}
\vspace{1em}
\setlength{\tabcolsep}{0.6em}
\label{tab:stat-defen}

\resizebox{\textwidth}{!}{

\begin{tabular}{cccccccc}
\hline
\makecell{ Detect \\type } & \makecell { Detect \\Name }  & \text{Year} &  \makecell { Defensive \\targets} &  \makecell {Adversary \\assumption}  &  \makecell{Main-task \\degradation}  &  \makecell{Data \\distribution} &  \makecell{Application}\\

\hline
\multicolumn{1}{c}{\multirow{5}{*}{Pre-AD}} & FLAME~\cite{nguyen2022flame} & 2022 & Dynamic Attacks & - & \makecell{Reddit/ CIFAR10\\ IoT-Traffic} & non-IID & \makecell{IoTD\\ IC/ NWP}        \\ \cmidrule(l){2-8}
\multicolumn{1}{c}{} & Flguard~\cite{nguyen2021flguard} & 2021 & Label-flipping & \makecell{knowledge of the \\ aggregator’s operations} & \makecell{Reddit/ CIFAR-10} & non-IID/ IID & IC/ NWP              \\ \cmidrule(l){2-8}
\multicolumn{1}{c}{} & VAE~\cite{li2020learning} & 2020 & \makecell{Label-flipping\\ Single-trigger} & \makecell{stale whitebox \\model inspection } & \makecell{MNIST, FEMNIST\\ Sentiment140} & non-IID & IC/ SA               \\ \cmidrule(l){2-8}
\multicolumn{1}{c}{} & FoolsGold~\cite{fung2018mitigating} & 2018 & Label-flipping & \makecell{knowledge of the \\total averaged gradient} & MNIST & non-IID & IC                   \\ \cmidrule(l){2-8}
\multicolumn{1}{c}{} & AUROR~\cite{shen2016auror} & 2016 & Label-flipping & - & MNIST/ GTSRB & IID & IC                   \\ \hline
\multicolumn{1}{c}{\multirow{8}{*}{In-AD}} & CRFL~\cite{xie2021crfl} & 2021 & Distributed-trigger & - & \makecell{LOAN/ EMNIST\\ MNIST} & non-IID & B\&F/ IC             \\ \cmidrule(l){2-8}
\multicolumn{1}{c}{} & BaFFle~\cite{andreina2021baffle} & 2021 & Label-flipping & \makecell{a number of \\compromised clients} & CIFAR-10/ FEMNIST & non-IID & IC                   \\ \cmidrule(l){2-8}
\multicolumn{1}{c}{} & RLR~\cite{ozdayi2021defending} & 2021 & Single-trigger & \makecell{limited adversarial \\client quantity} & CIFAR10 & IID & IC                   \\ \cmidrule(l){2-8}
\multicolumn{1}{c}{} & DP~\cite{bagdasaryan2020backdoor} & 2020 & Single-trigger & - & CIFAR/ Reddit & - & IC/ NLP              \\ \cmidrule(l){2-8}
\multicolumn{1}{c}{} & Optimised training~\cite{chen2020backdoor} & 2020 & Single-trigger & - & \makecell{ Omniglot\\ mini-Imagenet} & - & IC                   \\ \cmidrule(l){2-8}
\multicolumn{1}{c}{} & FL-WBC~\cite{sun2021fl} & 2020 & Label-flipping & - & \makecell{CIFAR10\\ FashionMNIST} & non-IID/ IID & IC                   \\ \cmidrule(l){2-8}
\multicolumn{1}{c}{} & FL-Pivot Training~\cite{zhang2020defending} & 2020 & Label-flipping & - & MNIST/ FMNIST & - & IC                   \\ \cmidrule(l){2-8}
\multicolumn{1}{c}{} & Weak DP/ Central DP~\cite{Sun2019CanYR} & 2019 & Single-trigger & \makecell{holding training samples\\ from the global distribution} & EMNIST & non-IID & IC                   \\ \hline
\multicolumn{1}{c}{\multirow{2}{*}{Post-AD}} & KD Unlearning~\cite{wu2022federated} & 2022 & Single-trigger & - & \makecell{MNIST/ CIFAR10\\ GTSRB} & - & IC                   \\ \cmidrule(l){2-8}
\multicolumn{1}{c}{} & Pruning Neurons~\cite{wu2020mitigating} & 2020 & Single-trigger & - & MNIST/ FashionMNIST & IID & IC                   \\

\hline
\multicolumn{3}{l}{NLP: Natural Language Processing}                                                                                             & \multicolumn{2}{l}{IoTD: IoT intrusion detection}    & \multicolumn{2}{l}{IC: Image Classification}                                                                              \\ 
\multicolumn{3}{l}{SA: Sentiment Analysis}                                                                                                       & \multicolumn{2}{l}{NWP: Next Word Prediction}        & \multicolumn{2}{l}{B\&F: Banking and Finance} \\ 
\end{tabular}
    
}
\end{table*}

==> tables/backdoor-defense-terminologies.tex <==
\begin{table*}[tbh]
\centering
\caption{BACKDOOR DEFENSES TERMINOLOGIES}

\tiny
\resizebox{\textwidth}{!}{
\begin{tabular}{cll}
\hline \hline
Terminology    & \multicolumn{1}{c}{Value}          & \multicolumn{1}{c}{Description}  \\ \hline
\multirow{3}{*}{Detect type} & Pre-AD   &  Identify misbehaving clients in FL settings before training process\\ 
                             & In-AD     & \makecell{Replace standard aggregation by a more robust one to alleviate the \\impact of malicious clients on global model.} \\ % (Robust Federated training, Differential Privacy)}  \\
                             & Post-AD &  Repair a backdoored global model after training process\\ \hline
Defensive targets            &  & What specific categories of backdoor attack does this defense address?  \\ \hline
Adversary assumption         & Training configuration/ Model Architecture/ Data distribution & How does the attacker know the training model/ process or data?\\ \hline
Main-task degradation   & High/ Medium/ Low  & How will main task accuracy decrease? \\ \hline
Data distribution            & IID/ non-IID; Hetero/ Homo & How is this defense's data division setup?\\ \hline
Defense effectiveness       & Reduce/ Eliminate & What is the effectiveness of this defense?\\ \hline
Application fields           & \makecell{Heathcare/ Smart Cities/ Autonomous Industry/ \\ NLP/ Banking and Finance/ Edge Computing and IoT \\ Computer Vision/ Nature Language Processing\\ Automatic Speech Recognition/ Healthcare/ Blockchain } & Which fields is this defense applicable for?\\ \hline
% / Biomedical and Industrial Management
\end{tabular}}
\end{table*}


==> tables/related-survey-back.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\renewcommand{\arraystretch}{1.25}
% \begin{table}[tbh]
% \scriptsize
% \centering
% \caption{Summary table of survey papers and main focus}
% \vspace{1em}
% \label{tab:survey-summary}
% \resizebox{0.9\textwidth}{!}{
% \begin{tabular}{@{}cp{0.15\textwidth 
%  }cccccc@{}}
% \toprule
% \multirow{2}{*}{Survey paper} & \multirow{2}{*}{Summary} & \multicolumn{4}{c}{Main focus} & \multicolumn{2}{c}{Applicable field} \\ \cmidrule(l){3-6} \cmidrule(l){7-8} 
%   &                          & \begin{tabular}[c]{@{}c@{}}Privacy/Security \\ threats\end{tabular} & \begin{tabular}[c]{@{}c@{}}Poisoning\\ attacks\end{tabular} & \begin{tabular}[c]{@{}c@{}}Backdoor \\ attacks\end{tabular} & \begin{tabular}[c]{@{}c@{}}Corresponding\\countermeasures \end{tabular}& ML                & FL               \\ \midrule

% \cite{Chen2017TargetedBA} & Backdoor poisoning attacks & & & \checkmark & & \checkmark & \\
% \cite{Miller2020AdversarialLT} & Defenses against adversarial learning attacks & & \checkmark &  &  & \checkmark & \\
% \cite{Goldblum2022-wq} & Data poisoning attacks & & \checkmark & & & \checkmark &\\
% \cite{Li2022BackdoorLA} & Backdoor attack and defenses & & & \checkmark & \checkmark & \checkmark & \checkmark \\
% \cite{Tian2022ACS} & Poisoning attacks and countermeasures & & \checkmark &  & & \checkmark & \checkmark\\
% \cite{Abdulrahman2021ASO} & FL challenges, contributions, and trends & \checkmark & & & & & \checkmark\\
% \cite{Yin2021ACS} & Privacy-preserving FL & \checkmark & & & & &  \checkmark\\
% \cite{Mothukuri2021ASO} & Security and Privacy in FL & \checkmark & & & & &  \checkmark \\
% \cite{Gosselin2022PrivacyAS} & FL security and privacy threats & \checkmark & & & & & \checkmark \\
% \cite{Lyu2020ThreatsTF} & Threats and attacks in FL & \checkmark & \checkmark & \checkmark & \checkmark & & \checkmark\\
% \cmidrule(l){1-8}
% \textbf{Ours} & Backdoor attacks and countermeasures in FL &  &  & \checkmark & \checkmark & & \checkmark\\
% \bottomrule
% \end{tabular}
% }
% \end{table}

\begin{table}[tbh]
% \scriptsize
\centering
\caption{{A Summary of Existing Surveys Related to FL Backdoor Attacks \textcolor{purple}{TODO: Add BD defense columns}}}
\vspace{1em}
\label{tab:survey-summary}
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{@{}p{0.3\textwidth}ccccccccccc@{}}
\toprule
         &  
         & \multicolumn{3}{c}{Main focus}                                   
    & \multicolumn{3}{c}{FL \textcolor{red}{category}}                         
                & \multicolumn{4}{c}{Survey methodology}                                
\\ \cmidrule(l){3-5} \cmidrule(l){6-8} \cmidrule(l){9-12}
                            %   \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Survey\\paper\end{tabular}} 
\multicolumn{1}{c}{Survey paper} & Year 
% &\multicolumn{1}{l}{Summary}                     
        & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Privacy/security \\ threats\end{tabular}} 
        & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Poisoning\\ attacks\end{tabular}}
        & \begin{tabular}[c]{@{}c@{}}Backdoor \\ attacks\end{tabular} 
        
    % & \multicolumn{1}{c}{ML} 
    & \multicolumn{1}{c}{HFL} 
    & VFL 
    & FTL
                & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Technique\\ driven\end{tabular}} 
                & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Inter\\connection\end{tabular}} 
                & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Evaluation \\ metrics\end{tabular}} 
                & \begin{tabular}[c]{@{}c@{}} Backdoor\\ applicability\end{tabular} \\ \midrule
                
Data poisoning attacks\cite{Goldblum2022-wq} & 2022 &  & \checkmark & & \checkmark & & & \checkmark & & & \checkmark\\
 Backdoor attack and defenses\cite{Li2022BackdoorLA} & 2022 & & & \checkmark & &  &  & \checkmark & & \checkmark & \checkmark\\
 Backdoor Attacks and Defenses in FL\cite{ba-fl-survey-2022} & 2022 & &  & \checkmark & \checkmark & & & \checkmark &\\
% \cite{Tian2022ACS} & Poisoning attacks and countermeasures & & \checkmark &  & & \checkmark & \checkmark\\
Poisoning attacks and countermeasures\cite{Tian2022ACS} & 2022 & & \checkmark & & \checkmark & & &\checkmark & \checkmark & \checkmark & \checkmark \\
FL challenges, contributions, and trends\cite{Abdulrahman2021ASO} & 2021  & \checkmark & & & \checkmark & \checkmark & \checkmark &\checkmark\\
 Privacy-preserving FL\cite{Yin2021ACS} & 2021 & \checkmark & & & \checkmark & \checkmark &  \checkmark & \checkmark\\
 Security and Privacy in FL\cite{Mothukuri2021ASO} & 2021 & \checkmark & & & & \checkmark &  \checkmark & \checkmark \\
 FL security and privacy threats\cite{Gosselin2022PrivacyAS} & 2022 & \checkmark & & & \checkmark & \checkmark &  \checkmark & \checkmark \\
 Threats and attacks in FL\cite{Lyu2020ThreatsTF} & 2020 & \checkmark &  &  &  & \checkmark & \checkmark & \checkmark & \checkmark & & \\                                               
&                                                                   \\ 
 
  Backdoor poisoning attacks\cite{Chen2017TargetedBA} & 2017 & & &  & \checkmark & & & \checkmark & & & \checkmark\\
  
\cmidrule(l){1-12}
\multicolumn{2}{c}{\textbf{Ours}} & & & \checkmark &  \checkmark  & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark\\
\bottomrule
\multicolumn{3}{l}{HFL: Horizontal Federated Learning} & \multicolumn{5}{l}{VFL: Vertical Federated Learning}      & \multicolumn{3}{l}{FTL: Federated Transfer Learning}      &    \\    
\end{tabular}
}
\end{table}

==> tables/survey-summary.tex <==

\begin{table*}[hbt!]
\scriptsize
\centering
\caption{Summary table of survey papers and main focus}
\vspace{1em}
\label{tab:survey-summary}
\resizebox{0.9\textwidth}{!}{
%     \begin{tabular}{c p{0.6\textwidth} p{0.15\textwidth}}
%     \toprule \hline \text { Survey paper } & \text{Summary} & \makecell { Main Focus } \\
%     \hline
%     \cite{Yin2021ACS} & Analyze the privacy leakage risks in the FL from five aspects, summarize existing methods, and identify future research directions & Privacy-preserving FL \\
%         \cite{Mothukuri2021ASO} & Review of security and privacy concerns that need to be considered in a thorough and clear context of FL & Security and Privacy in FL \\
%     \cite{Lyu2020ThreatsTF} & A concise introduction to the concept of FL, taxonomy and key techniques of threat models on FL and promising future research directions towards more robust privacy preservation in FL & Threats and attacks in FL \\
%     \cite{Chen2017TargetedBA} & Study different data poisoning strategies to perform backdoor attacks in ML & Backdoor poisoning attacks\\
%     \cite{Miller2020AdversarialLT} & Provide a contemporary
% survey of Adversarial Learning with main focus on corresponding defenses against attacks on deep neural network classifiers & Defenses against adversarial learning attacks\\
%     \cite{Li2022BackdoorLA} & Summarize
% and categorize existing backdoor attacks and defenses based
% on their characteristics, and provide a unified framework for
% analyzing poisoning-based backdoor attacks & Backdoor attack and defenses\\
%     \cite{Goldblum2022-wq} & Catalog and systematize vulnerabilities in the dataset creation process, which lead to data poisoning or dataset tampering in ML & Data poisoning attacks\\
%     \cite{Abdulrahman2021ASO} & Comprehensive taxonomies covering challenges, contributions, and trends of FL including core system models and designs, application areas, privacy and security, and resource management & FL challenges, contributions, and trends\\
%     \cite{Gosselin2022PrivacyAS} & Discuss the major security threats/attacks, FL-based solutions counteracting theses threats and ongoing research directions & FL  security and privacy threats\\
%     \cite{Liu2022ThreatsAA} & Systematically present the threats, attacks and defenses to FL throughout the whole process of FL in three phases, including Data and Behavior Auditing Phase, Training Phase and Predicting Phase & Threats and defenses in multi-phases of FL \\
%     \cite{Tian2022ACS} & Provide a unified perspective poisoning attacks and countermeasures: analysis, challenges and potential directions for both FL and ML & Poisoning attacks and countermeasures \\
%     \hline \bottomrule
%     \end{tabular}
\renewcommand{\arraystretch}{1.5}
\begin{tabular}{@{}c p{0.55\textwidth}p{0.15\textwidth}@{}}
\toprule \specialrule{0.4pt}{1pt}{1pt}
\multicolumn{2}{c}{Survey Paper} &
% \multicolumn{1}{c}{Summary}    
& Main Focus                                                              \\ \midrule
    \cite{Chen2017TargetedBA} & Study different data poisoning strategies to perform backdoor attacks in ML & Backdoor poisoning attacks\\
    \cite{Miller2020AdversarialLT} & Provide a contemporary
survey of Adversarial Learning with main focus on corresponding defenses against attacks on deep neural network classifiers & Defenses against adversarial learning attacks\\
    \cite{Goldblum2022-wq} & Catalog and systematize vulnerabilities in the dataset creation process, which lead to data poisoning or dataset tampering in ML & Data poisoning attacks\\
    \cite{Li2022BackdoorLA} & Summarize and categorize existing backdoor attacks and defenses based
on their characteristics, and provide a unified framework for
analyzing poisoning-based backdoor attacks & Backdoor attack and defenses\\
    \cite{Tian2022ACS} & Provide a unified perspective poisoning attacks and countermeasures: analysis, challenges and potential directions for both FL and ML & Poisoning attacks and countermeasures \\
    \cite{Abdulrahman2021ASO} & Comprehensive taxonomies covering challenges, contributions, and trends of FL including core system models and designs, application areas, privacy and security, and resource management & FL challenges, contributions, and trends\\
    \cite{Yin2021ACS} & Analyze the privacy leakage risks in the FL from five aspects, summarize existing methods, and identify future research directions & Privacy-preserving FL \\
    \cite{Mothukuri2021ASO} & Review of security and privacy concerns that need to be considered in a thorough and clear context of FL & Security and Privacy in FL \\
    \cite{Gosselin2022PrivacyAS} & Discuss the major security threats/attacks, FL-based solutions counteracting theses threats and ongoing research directions & FL security and privacy threats\\
    \cite{Lyu2020ThreatsTF} & A concise introduction to the concept of FL, taxonomy and key techniques of threat models on FL and promising future research directions towards more robust privacy preservation in FL & Threats and attacks in FL \\
            %  & \begin{tabular}[c]{@{}l@{}}Analyze the privacy leakage risks in the FL from five aspects, summarize existing methods, and identify future research directions\end{tabular}                                                      & Privacy-preserving FL                                                   \\
            %  & \begin{tabular}[c]{@{}l@{}}Review of security and privacy concerns that need to be considered in a thorough and clear context\\ \\ of FL\end{tabular}                                                                                & \begin{tabular}[c]{@{}c@{}}Security and Privacy in\\ \\ FL\end{tabular} \\
            %  & \begin{tabular}[c]{@{}l@{}}A concise introduction to the concept of FL, taxonomy and key techniques of threat models on FL\\ \\ and promising future research directions towards more robust privacy preservation in FL\end{tabular} & Threats and attacks in FL                                               \\ \bottomrule
        \specialrule{0.4pt}{1pt}{1pt}
        \bottomrule
\end{tabular}}
\end{table*}

==> tables/works-on-backdoor-attacks.tex <==
% \begin{table*}[hbt!]
% \scriptsize
% \centering
% \caption{Annual Distribution of Backdoor Attack-related Papers in FL and ML from Google Scholar}
% \vspace{1em}
% \setlength{\tabcolsep}{0.6em}
% \label{tab:stat-defen}

% \resizebox{\textwidth}{!}{

%     \begin{tabular}{lcccc}
%     \hline
%     Year        & Backdoor Attack in ML & Backdoor Attack in FL & Backdoor Defense in ML & Backdoor Defense in FL  \\
%     \hline 2015        & 2420                                & 0                                     \\
%     2015 → 2016 & 4980                                & 0                                     \\
%     2015 → 2017 & 7590                                & 0                                     \\
%     2015 → 2018 & 10400                               & 15                                    \\
%     2019 → 2019 & 13600                                & 79                                    \\
%     2019 → 2020 & 15700                                & 384                                   \\
%     2019 → 2021 & 16100                               & 1040                                  \\
%     2019 → 2022 & 15100                               & 2130                                  \\
%     Since 2023  & 297                                 & 71 \\                   \hline
%     \end{tabular}
% }

% \end{table*}
\begin{figure}[tbh]
    \centering
    \includegraphics[width=0.4\textwidth]{figures/paper_counting.pdf}
    \caption{Frequency of backdoor-related keywords appeared on titles or abstracts of publications by \textit{app.dimensions.ai}. \textit{Note}: The data was collected on 1 February 2023.}
    \label{fig:count_works}
\end{figure}
